Pyrometheus: Symbolic abstractions for XPU and automatically differentiated computation of combustion kinetics and thermodynamics

The cost of combustion simulations is often dominated by the evaluation of net production rates of chemical species and mixture thermodynamics (thermochemistry). Execution on computing accelerators (XPUs) like graphic processing units (GPUs) can greatly reduce this cost. However, established thermochemistry software is not readily portable to such devices or sacrifices valuable analytical forms that enable differentiation for sensitivity analysis and implicit time integration. Symbolic abstractions are developed with corresponding transformations that enable computation on accelerators and automatic differentiation by avoiding premature specification of detail. The software package Pyrometheus is introduced as an implementation of these abstractions and their transformations for combustion thermochemistry. The formulation facilitates code generation from the symbolic representation of a specific thermochemical mechanism in multiple target languages, including Python, C++, and Fortran. Computational concerns are separated: the generated code processes array-valued expressions but does not specify their semantics. These semantics are provided by compatible array libraries, such as NumPy, Pytato, and Google JAX. Thus, the generated code retains a symbolic representation of the thermochemistry, which translates to computation on accelerators and CPUs and automatic differentiation. The design and operation of these symbolic abstractions and their companion tool, Pyrometheus, are discussed throughout. Roofline demonstrations show that the computation of chemical source terms within MFC, a Fortran-based flow solver we link to Pyrometheus, is performant.

==> Figures/MFC/tex/weak_scaling_frontier.tex <==
%! TEX root=weak_scaling_frontier.tex
\input{tikz_preamble.tex}

\pagestyle{empty}
\begin{document}

\begin{tikzpicture}
    \begin{axis}[
        xmode = log, 
        ylabel style={align=center},
        xlabel = {Number of MI250X GCDs},
        ylabel = {Normalized Wall Time},
        axis background/.style={},
        ticklabel style={},
        label style={},
        width = 3.5in,
        height = 1.75in, 
        xmin=80,
        xmax=200000,
        ymin = 0, 
        ymax = 1.5,
        legend style={at={(0,0)}, anchor=south west,draw=none,fill=none,inner sep=5pt,legend columns=2,column sep=5pt},
    ]
        \addplot[black,dashed,thick,domain=80:75264] {1};
        \addplot[RYB2,thick,mark=*,mark size=2.2,only marks] 
            coordinates {
                (128,1.0) (384,1.004034) (1024,1.019502) (3072,1.021183) (8192,1.023874) (24576,1.039340) (65536, 1.047411)
            };
            %coordinates {
              %  (216,1) (432,0.9998799274) (864,1.008840948) (1728,1.008840948) (3456,1.024239052) (6912,1.019016381) (13824,1.028153615)
            %};
        \legend{Ideal,\color{RYB2}MFC};
        \draw[ultra thick,RYB1] (axis cs:75264,0) -- (axis cs:75264,1.5);
        \node[anchor=west,inner sep=2pt] at (axis cs:75264,0.75) 
            {\rotatebox{90}{\small\color{RYB1}100\% Frontier}};
        \draw[fill=black,opacity=0.08] 
            (axis cs:75264,0) rectangle (axis cs:200000,1.5); 

        %\draw[ultra thick,RYB1] (axis cs:75264,0) -- (axis cs:75264,1.5);
        %\node[anchor=west,inner sep=2pt] at (axis cs:75264,0.75) 
        %    {\rotatebox{90}{\footnotesize\color{RYB1}100\% Summit}};
        %\draw[fill=black,opacity=0.08] 
        %    (axis cs:75264,0) rectangle (axis cs:200000,1.5); 
    \end{axis}
\end{tikzpicture}

\end{document}


==> Figures/MFC/tikz_preamble.tex <==
\usepackage{bm}
\newcommand{\ve}[1]{\bm{#1}}

\newcommand{\ba}{\ve{a}}
\newcommand{\bb}{\ve{b}}
\newcommand{\bA}{\ve{A}}
\newcommand{\bu}{\ve{u}}
\newcommand{\bv}{\ve{v}}
\newcommand{\br}{\ve{r}}
\newcommand{\bp}{\ve{p}}
\newcommand{\bt}{\ve{t}}
\newcommand{\bn}{\ve{n}}
\newcommand{\bc}{\ve{c}}
\newcommand{\bq}{\ve{q}}
\newcommand{\bff}{\ve{f}}
\newcommand{\bx}{\ve{x}}
\newcommand{\by}{\ve{y}}
\newcommand{\be}{\ve{e}}
\newcommand{\bg}{\ve{g}}
\newcommand{\bs}{\ve{s}}

\newcommand{\bP}{\ve{P}}
\newcommand{\bS}{\ve{S}}
\newcommand{\bB}{\ve{B}}
\newcommand{\bU}{\ve{U}}
\newcommand{\bG}{\ve{G}}
\newcommand{\bV}{\ve{V}}
\newcommand{\bR}{\ve{R}}
\newcommand{\bQ}{\ve{Q}}
\newcommand{\bX}{\ve{X}}
\newcommand{\bC}{\ve{C}}
\newcommand{\bI}{\ve{I}}

\newcommand{\hx}{\hat{x}}
\newcommand{\hbx}{\ve{e}_x}
\newcommand{\hbr}{\ve{e}_r}

\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bEps}{\boldsymbol{\varepsilon}}
\newcommand{\beps}{\boldsymbol{\varepsilon}}
\newcommand{\bdelta}{\boldsymbol{\delta}}

\newcommand{\heps}{\hat{\varepsilon}}
\newcommand{\barx}{\widetilde{\ve{x}}}
\newcommand{\bara}{\widetilde{\ve{a}}}

\newcommand{\vq}{\vec{q}}
\newcommand{\vba}{\vec{\ve{a}}}
\newcommand{\vbu}{\vec{\ve{u}}}
\newcommand{\vbx}{\vec{\ve{x}}}
\newcommand{\vby}{\vec{\ve{y}}}
\newcommand{\vbv}{\vec{\ve{v}}}
\newcommand{\vbr}{\vec{\ve{r}}}
\newcommand{\vbs}{\vec{\ve{s}}}
\newcommand{\vblambda}{\vec{\boldsymbol{\lambda}}}
\newcommand{\vbsigma}{\vec{\boldsymbol{\sigma}}}
\newcommand{\vbEps}{\vec{\boldsymbol{\varepsilon}}}
\newcommand{\vbdelta}{\vec{\boldsymbol{\delta}}}

\newcommand{\eps}{\varepsilon}
\newcommand{\dd}{\text{d}}
\newcommand{\gdot}{\dot\gamma}

\newcommand{\etal}{\textit{et al.\ }}

\newcommand\Rey{\mbox{\textit{Re}}}  % Reynolds number
\newcommand\Ca{\mbox{\textit{Ca}}} % Capillary number

\usepackage{amsmath}
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{bbm}
\usepackage{tikz}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\usepackage{natbib}
\usepackage{mhchem}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{quantikz}
\usetikzlibrary{arrows.meta, decorations.markings, positioning, quotes, shapes.arrows}
\usepackage[utf8]{inputenc}
\usepackage{siunitx}
\usepackage{xfrac}
\usepgfplotslibrary{colormaps}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.17}
\usepackage[html]{xcolor} 
\definecolor{omegaPos}{HTML}{0000FF}
\definecolor{omegaNeg}{HTML}{00AA00}
\usetikzlibrary{arrows.meta}
\textwidth = 6.5 in
\textheight = 8 in

\definecolor{RYB1}{RGB}{207, 37, 37}
\definecolor{RYB2}{RGB}{37, 91, 207}
\definecolor{RYB3}{RGB}{37, 207, 91}
\definecolor{RYB4}{RGB}{163,26,145}
\definecolor{RYB5}{RGB}{253, 180, 98}
\definecolor{RYB6}{RGB}{179, 222, 105}
\definecolor{RYB7}{RGB}{128, 177, 211}

\usepackage{xcolor}
\definecolor{lightblue}{rgb}{0.63, 0.74, 0.78}
\definecolor{seagreen}{rgb}{0.18, 0.42, 0.41}
\definecolor{orange}{rgb}{0.85, 0.55, 0.13}
\definecolor{silver}{rgb}{0.69, 0.67, 0.66}
\definecolor{rust}{rgb}{0.72, 0.26, 0.06}
\definecolor{purp}{RGB}{68, 14, 156}

\colorlet{lightrust}{rust!50!white}
\colorlet{lightorange}{orange!25!white}
\colorlet{lightlightblue}{lightblue}
\colorlet{lightsilver}{silver!30!white}
\colorlet{darkorange}{orange!75!black}
\colorlet{darksilver}{silver!65!black}
\colorlet{darklightblue}{lightblue!65!black}
\colorlet{darkrust}{rust!85!black}
\colorlet{darkseagreen}{seagreen!85!black}


\pgfplotscreateplotcyclelist{newcolors}{
{RYB1,every mark/.append style={fill=RYB1,mark size={2.5}},mark=*},
{RYB2,every mark/.append style={fill=RYB2},mark=square*},
{RYB3,every mark/.append style={fill=RYB3,mark size={3}},mark=triangle*},
{RYB4,every mark/.append style={fill=RYB4,mark size={3}},mark=diamond*},
{RYB5,every mark/.append style={fill=RYB5,mark size={3}},mark=pentagon*},
{RYB6,every mark/.append style={fill=RYB6,mark size={4}},mark=10-pointed star},
{RYB7,every mark/.append style={fill=RYB7},mark=*},
}

\pgfplotsset{
    standard/.style={
    	compat=1.18,
        scale only axis,
        width=0.5\textwidth,
        enlarge x limits=0.05,
        enlarge y limits=0.05,
        max space between ticks=40,
	    cycle list name=newcolors,
        every axis/.append style={font=\small},
        every legend/.append style={font=\small},
        every node/.append style={font=\small},	
	}
    every axis/.append style={font=\small},
    every legend/.append style={font=\small},
    every node/.append style={font=\small},	
}

\tikzset{
    every node/.append style={font=\small},	
}


==> Figures/fig-macros.tex <==

%\usepackage[dvipsnames]{xcolor}
\usepackage{tikz}
\usepackage{stackrel}
\usepackage{bm,bbm}% bold math
\usepackage[version=3]{mhchem}

\usepackage{multirow}
\usepackage{setspace}
\usepackage{yfonts}
\usepackage{mathrsfs}
%\usepackage{tcolorbox}
%\usepackage{colortbl}
\usepackage{commath}
\usepackage{algpseudocode}
\usepackage{xfrac}
\usepackage{mathtools}
\usepackage{empheq}

\usepackage{pgffor}
\usepackage{subfig}
\usepackage{standalone}
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots,units,external,fillbetween}
\usetikzlibrary{spy,arrows,arrows.meta,shapes,matrix,fit,backgrounds,calc,positioning}
\pgfplotsset{compat=newest}

\usepackage[colorinlistoftodos, color=blue!20!white, bordercolor=gray,
textsize=tiny]{todonotes}

\usepackage{amsmath,amsfonts,amssymb,amsthm,mathrsfs,mathtools}

%\setbeamercolor{structure}{fg=pdcolor2}
%\setbeamercolor{normal text}{fg=pdcolor1}

\usepackage{pgf}
\usetikzlibrary{arrows,shapes,shapes.arrows,positioning,calc,decorations.text,automata}

\usepackage{standalone}

\usepackage{pgfgantt}

\usepackage{multimedia}
\usepackage{graphicx}

\definecolor{grayish}{RGB}{35, 31, 32}
\definecolor{pdcolor1}{RGB}{51,51,102}  %UIUC blue (Formal Palette)
\definecolor{pdcolor2}{RGB}{204,102,0}  %UIUC orange (Formal Palette)
\definecolor{myTan}{RGB}{205,133,63}
\definecolor{myBrown}{RGB}{155,77,40}

\newcommand{\mynote}[1]{{\color{green} \tiny #1}}
\newcommand{\prj}[2]{{\color{gray} #1 [#2]}}
\newcommand{\talkref}[2]{{\color{gray} #1 [#2]}}
\newcommand{\makered}[1]{{\color{red} #1}}

\newcommand{\myoul}[1]{\color{pdcolor2}\underline{\smash{\color{pdcolor1} #1}}\color{pdcolor1}}
\newcommand{\ccdot}{\color{pdcolor2}$\circ$\color{pdcolor1}\;}
\newcommand{\cc}[1]{\color{pdcolor2}#1\color{pdcolor1}{}}

\newcommand{\HRule}[2]{{\color{pdcolor2}\rule{#1}{#2}}}
\newcommand{\dRightarrow}{{\color{pdcolor2}\Rightarrow}}
\newcommand{\dLeftarrow}{{\color{pdcolor2}\Leftarrow}}
\newcommand{\tb}[1]{{\color{blue}(#1)}}
\newcommand{\tr}[1]{{\color{blue}({\color{red}#1})}}
\newcommand{\tor}[1]{{\color{blue}({\color{blue}#1})}}
\newcommand{\lead}[1]{\textit{\color{pdcolor2}(#1)}}
\newcommand{\bmath}{\boldsymbol}
\newcommand{\eps}{\varepsilon}
\newcommand{\vp}{\vec{p}}
\newcommand{\rPI}[1]{{\color{pdcolor2}#1}}
\newcommand{\tPI}[1]{\texttt{\color{pdcolor2}#1}}
\newcommand{\cPI}[1]{\textbf{\color{pdcolor2}#1}}
\newcommand{\iPI}[1]{\textit{\color{pdcolor2}#1}}
\newcommand{\sPI}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\scPI}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\tabtit}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\Dpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\II}{{I\!I}}
\newcommand{\memph}[1]{{\color{red} #1}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand\ign{\mathrm{ign}}
\newcommand\tign[1]{\tau_{\ign}^{#1}}
\newcommand\btign[1]{\bvec{\tau}_{\ign}^{#1}}
\newcommand\bkappa{\bvec{\kappa}}


\newcommand\solidrule[1][0.75cm]{\rule[0.5ex]{#1}{.4pt}}
\newcommand\shortsolidrule[1][0.5cm]{\rule[0.5ex]{#1}{.4pt}}
\newcommand\thicksolidrule[1][0.5cm]{\rule[0.5ex]{#1}{.8pt}}
\newcommand\dashedrule{\mbox{%
    \solidrule[2mm]\hspace{2mm}\solidrule[2mm]\hspace{2mm}\solidrule[2mm]}}

\newcommand{\sectionWithFrame}[1]{%
  \section{#1}
  \begin{frame}
    \centerline{\LARGE \insertsection}
  \end{frame}}
\newcommand{\sectionAndsubWithFrame}[2]{%
  \section{#1}
  \begin{frame}
    \centerline{\LARGE \insertsection}
    \bigskip
    \centerline{\large #2}
  \end{frame}}

\newcommand{\cM}{\mathcal{M}}

\newcommand{\bn}{\mathbf{n}}

\newcommand{\bbC}{\mathbb{C}}
\newcommand{\vbbm}{{\vec{m}}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbV}{\mathbb{V}}

\newcommand{\vD}{{\vec D}}
\newcommand{\vhD}{{\hat{D}}}
\newcommand{\vg}{{\vec g}}
\newcommand{\vphi}{{\vec\phi}}
\newcommand{\vOmega}{{\vec\Omega}}

\newcommand{\vF}{{\vec{F}}}
\newcommand{\vf}{{\vec{f}}}
\newcommand{\vb}{{\vec{b}}}
\newcommand{\vq}{{\vec{q}}}
\newcommand{\vqs}{{\vec{q}^{\,\color{red}*}}}

\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\rstar}{{\color{red}*}}
\newcommand{\rchk}{{\color{red} \checkmark}}
\newcommand{\gchk}{{\color{green} \checkmark}}
\newcommand{\rbul}{{\color{red} $\bullet$}}
\newcommand{\pbul}{{\color{pdcolor2} $\bullet$}}
\newcommand{\ro}{{\color{red} $\circ$}}
\newcommand{\bd}{{\color{blue} $\bullet$}}

\newcommand{\rhoi}[1][i]{\rho_{#1}}
\newcommand{\dt}[1][t]{\partial_{#1}}
\newcommand{\dx}[1][{\textrm{\bf x}}]{\boldsymbol \partial_{#1}}
\newcommand{\Vi}[1][i]{\mathcal{V}_{#1}}
\newcommand{\Mi}[1][\textswab{i}]{\mathcal{M}_{#1}}
\newcommand{\omegai}[1][i]{\dot{\omega}_{#1}}
\newcommand{\grav}{{\bf g}}
\newcommand{\Etot}{\mathcal{E}}

\newcommand{\mBG}{m_{\text{\tiny BG}}}
\newcommand{\nBG}{n_{\text{\tiny BG}}}
\newcommand{\nIp}{n_{\text{\tiny $I^+$}}}
\newcommand{\nIm}{n_{\text{\tiny $I^-$}}}


\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\btau}{{\boldsymbol{\tau}}}

\newcommand{\bv}{{\bar{v}}}
\newcommand{\bepsilon}{{\bar{\epsilon}}}

\newcommand{\ST}{{S_{\text{\tiny T}}}}

\newcommand{\vu}{\vec{u}}
\newcommand{\vQ}{\vec{Q}}
\newcommand{\veta}{\vec{\eta}}


\newcommand{\Grad}{\bnabla}
\newcommand{\Div}{\bnabla\vdot}
\newcommand{\Curl}{\bnabla\vprod}
\newcommand{\hGrad}{\bnabla^{}_{\!\!\mathrm{h}}}
\newcommand{\hDiv}{\bnabla^{}_{\!\!\mathrm{h}}\!\vdot}
\newcommand{\pGrad}{\bnabla^{}_{\!\!\!\perp}}
\newcommand{\pDiv}{\bnabla^{}_{\!\!\!\perp}\!\vdot}
\newcommand{\pop}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pp}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\psq}[1]{\ensuremath{{\left[ #1 \right]}}}
\newcommand{\pcr}[1]{\ensuremath{\left\{ #1 \right\}}}

% Grad, div, curl, etc.
\newcommand{\vdot}{\mathop{\mbox{\boldmath{$\cdot$}}}}
\newcommand{\vddot}{\mathop{\mbox{\textbf{:}}}}
\newcommand{\bnabla}{\mbox{\boldmath{$\nabla$}}}
\newcommand{\Lapl}{\nabla^2}
\newcommand{\hLapl}{\nabla^2_{\!\mathrm{h}}}
\newcommand{\pLapl}{\nabla^2_{\!\!\!\perp}}

\newcommand{\kION}{k_{\text{\tiny ION}}}
\newcommand{\kDET}{k_{\text{\tiny DET}}}
\newcommand{\kDR}{k_{\text{\tiny DR}}}
\newcommand{\kDA}{k_{\text{\tiny DA}}}
\newcommand{\kII}{k_{\text{\tiny $II$}}}


\def\colorize<#1>{%
\temporal<#1>{}{\color{red}}{}
}

\newcommand{\TODO}[1]{{\color{pink} \tiny TODO: #1}}
\newcommand{\CHK}{{\color{red} ???}}
\newcommand{\progname}[1]{\textit{#1}}
\newcommand{\PlasComCM}{\progname{PlasComCM}}
\newcommand{\PlasComCMtwo}{\progname{PlasCom2}}
\newcommand{\dancode}{\PlasComCM}
\newcommand{\dancodetwo}{\progname{PlasCom2}}
\newcommand{\codelet}[1]{\progname{Codelet-#1}}
\newcommand{\goldenCopy}{\rPI{golden copy}}
\newcommand{\GoldenCopy}{\rPI{Golden copy}}
\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\Q}[1]{{\medskip\small\noindent\color{red}#1\par}}

\newcommand{\insertmovie}[3]{\ifmovies{
\movie[autostart,loop]
{\includegraphics[width=#1\textwidth]{Movies/#2}}
{Movies/#3}
}
\else{
\includegraphics[width=#1\textwidth]{Movies/#2}
}
\fi
}

\definecolor{ForestGreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{antiquewhite}{rgb}{0.98, 0.92, 0.84}

\newcommand{\MUST}{{\footnotesize\color{red} \textbf{MUST}}}
\newcommand{\WISH}{{\footnotesize\color{orange} \textbf{WISH}}}
\newcommand{\DEFER}{{\footnotesize\color{yellow} \textbf{DEFER}}}
\newcommand{\RETURN}{{\footnotesize\color{blue} \textbf{RETURN}}}
\newcommand{\DONE}{{\footnotesize\color{ForestGreen} \textbf{COMPLETED}}}
\newcommand{\PLAN}{{\footnotesize\color{green} \textbf{PLANNED}}}

\newcommand{\SNL}{{\footnotesize $\;\rightarrow$ SNL}}
\newcommand{\LLNL}{{\footnotesize $\;\rightarrow$ LLNL}}
\newcommand{\LANL}{{\footnotesize $\;\rightarrow$ LANL}}


\newcommand{\aMUST}{\tiny\raisebox{1.5pt}{\color{red} (\textbf{M})}}
\newcommand{\aWISH}{\raisebox{1.5pt}{\tiny\color{orange} (\textbf{W})}}
\newcommand{\aDEFER}{\raisebox{1.5pt}{\tiny\color{yellow} (\textbf{D})}}
\newcommand{\aRETURN}{\raisebox{1.5pt}{\tiny\color{blue} (\textbf{R})}}
\newcommand{\aDONE}{\raisebox{1.5pt}{\tiny\color{ForestGreen} (\textbf{C})}}
\newcommand{\aPLAN}{\raisebox{1.5pt}{\tiny\color{green} (\textbf{P})}}

\newcommand{\Resp}{\cPI{Response}}
\newcommand{\Recm}{\cPI{Recommendation}}


\newcommand{\recbox}[1]{
\fcolorbox{pdcolor2}{antiquewhite}{
\begin{minipage}{0.97\textwidth}
\noindent
\Recm:
{#1}
\end{minipage}}
}
\newcommand{\recb}[1]{\fcolorbox{pdcolor2}{antiquewhite}{\Recm: #1}}

\newcommand{\recboxnt}[1]{
\fcolorbox{pdcolor2}{antiquewhite}{
\begin{minipage}{0.97\textwidth}
{#1}
\end{minipage}}
}

%\arrayrulecolor{pdcolor2}

\usepackage{pgfplots}
\usepackage{pgfplotstable}

\definecolor{RYB1}{RGB}{207, 37, 37}
\definecolor{RYB2}{RGB}{37, 91, 207}
\definecolor{RYB3}{RGB}{37, 207, 91}
\definecolor{RYB4}{RGB}{163,26,145}
\definecolor{RYB5}{RGB}{253, 180, 98}
\definecolor{RYB6}{RGB}{179, 222, 105}
\definecolor{RYB7}{RGB}{128, 177, 211}
\definecolor{RYB8}{RGB}{203, 71, 119}
\definecolor{RYB9}{RGB}{200., 220., 231.333}

\definecolor{RED}{RGB}{255,0,0}  %%% 
\definecolor{myBlue}{RGB}{19,41,75}  %%% BLUE
\definecolor{myBlueLink}{RGB}{70,70,200}  %%% ILLINOIS BLUE
\definecolor{myOrange}{RGB}{232,74,39}   %%% ILLINOIS ORANGE
\definecolor{IllinoisOrange}{RGB}{232,74,39}  %%% ILLINOIS ORANGE
\definecolor{IllinoisBlue}{RGB}{19,41,75}   %%% ILLINOIS BLUE
\definecolor{mainTextColor}{RGB}{19,41,75}  %%% ILLINOIS BLUE
\definecolor{myLightGray}{rgb}{0.95,0.95,0.95} 

\pgfplotscreateplotcyclelist{newcolors}{
{RYB1,every mark/.append style={fill=RYB1,mark size={2.5}},mark=*},
{RYB2,every mark/.append style={fill=RYB2},mark=square*},
{RYB3,every mark/.append style={fill=RYB3,mark size={3}},mark=triangle*},
{RYB4,every mark/.append style={fill=RYB4,mark size={4}},mark=x},
{RYB5,every mark/.append style={fill=RYB5,mark size={3}},mark=oplus},
%{RYB6,every mark/.append style={fill=RYB6,mark size={4}},mark=10-pointed star},
{RYB7,every mark/.append style={fill=RYB7},mark=*},
}
\pgfplotsset{
  %  every axis/.append style={
 %       scale only axis,
 %      width=0.5\textwidth,
%    },
    standard/.style={
    thick,
    compat=1.8,
            scale only axis,
        width=0.45\textwidth,
  %      axis x line=middle,
%        axis y line=middle,
        enlarge x limits=0.05,
        enlarge y limits=0.05,
  %      every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
  %      every axis y label/.style={at={(current axis.above origin)},anchor=north east},
        max space between ticks=40,
 %       tick label style={font=\Large},
%label style={font=\Large},
%legend style={font=\Large},
cycle list name=newcolors
%    cycle list={RYB1\\RYB2\\RYB3\\RYB4\\RYB5}
    }
}

\definecolor{BluesA}{RGB}{247,251,255} % 0
\definecolor{BluesB}{RGB}{222,235,247} % 0.125
\definecolor{BluesC}{RGB}{198,219,239} % 0.250
\definecolor{BluesD}{RGB}{158,202,225} % 0.375
\definecolor{BluesE}{RGB}{107,174,214} % 0.500
\definecolor{BluesF}{RGB}{66,146,198}  % 0.625
\definecolor{BluesG}{RGB}{33,113,181}  % 0.750
\definecolor{BluesH}{RGB}{8,81,156}    % 0.875
\definecolor{BluesI}{RGB}{8,48,107}    % 1

\definecolor{SpectralA}{RGB}{94,79,162}   % 1
\definecolor{SpectralB}{RGB}{50,136,189}  % 0.9
\definecolor{SpectralC}{RGB}{102,194,165} % 0.8
\definecolor{SpectralD}{RGB}{171,221,164} % 0.7
\definecolor{SpectralE}{RGB}{230,245,152} % 0.6
\definecolor{SpectralF}{RGB}{255,255,191} % 0.5
\definecolor{SpectralG}{RGB}{254,224,139} % 0.4
\definecolor{SpectralH}{RGB}{253,174,97}  % 0.3
\definecolor{SpectralI}{RGB}{244,109,67}  % 0.2
\definecolor{SpectralJ}{RGB}{213,62,79}   % 0.1
\definecolor{SpectralK}{RGB}{158,1,66}    % 0

\definecolor{RdYlBuA}{RGB}{165,0,38}    % 0
\definecolor{RdYlBuB}{RGB}{215,48,39}   % 0.1
\definecolor{RdYlBuC}{RGB}{244,109,67}   % 0.2
\definecolor{RdYlBuD}{RGB}{253,174,97} % 0.3
\definecolor{RdYlBuE}{RGB}{254,224,144} % 0.4
\definecolor{RdYlBuF}{RGB}{255,255,191} % 0.5
\definecolor{RdYlBuG}{RGB}{224,243,248} % 0.6
\definecolor{RdYlBuH}{RGB}{171,217,233} % 0.7
\definecolor{RdYlBuI}{RGB}{116,173,209}  % 0.8
\definecolor{RdYlBuJ}{RGB}{69,117,180}  % 0.9
\definecolor{RdYlBuK}{RGB}{49,54,149}     % 1

\definecolor{RdBuA}{RGB}{103,0,31}    % 0
\definecolor{RdBuB}{RGB}{178,24,43}   % 0.1
\definecolor{RdBuC}{RGB}{214,96,77}   % 0.2
\definecolor{RdBuD}{RGB}{244,165,130} % 0.3
\definecolor{RdBuE}{RGB}{253,219,199} % 0.4
\definecolor{RdBuF}{RGB}{247,247,247} % 0.5
\definecolor{RdBuG}{RGB}{209,229,240} % 0.6
\definecolor{RdBuH}{RGB}{146,197,222} % 0.7
\definecolor{RdBuI}{RGB}{67,147,195}  % 0.8
\definecolor{RdBuJ}{RGB}{33,102,172}  % 0.9
\definecolor{RdBuK}{RGB}{5,48,97}     % 1

\definecolor{RdGyA}{RGB}{103,0,31}    % 0
\definecolor{RdGyB}{RGB}{178,24,43}   % 0.1
\definecolor{RdGyC}{RGB}{214,96,77}   % 0.2
\definecolor{RdGyD}{RGB}{244,165,130} % 0.3
\definecolor{RdGyE}{RGB}{253,219,199} % 0.4
\definecolor{RdGyF}{RGB}{255,255,255} % 0.5
\definecolor{RdGyG}{RGB}{224,224,224} % 0.6
\definecolor{RdGyH}{RGB}{186,186,186} % 0.7
\definecolor{RdGyI}{RGB}{135,135,135} % 0.8
\definecolor{RdGyJ}{RGB}{77,77,77}    % 0.9
\definecolor{RdGyK}{RGB}{26,26,26}    % 1

\definecolor{PuOrA}{RGB}{127,59,8}    % 0
\definecolor{PuOrB}{RGB}{179,88,6}   % 0.1
\definecolor{PuOrC}{RGB}{224,130,20}   % 0.2
\definecolor{PuOrD}{RGB}{253,184,99} % 0.3
\definecolor{PuOrE}{RGB}{254,224,182} % 0.4
\definecolor{PuOrF}{RGB}{247,247,247} % 0.5
\definecolor{PuOrG}{RGB}{216,218,235} % 0.6
\definecolor{PuOrH}{RGB}{178,171,210} % 0.7
\definecolor{PuOrI}{RGB}{128,115,172} % 0.8
\definecolor{PuOrJ}{RGB}{84,39,136}    % 0.9
\definecolor{PuOrK}{RGB}{45,0,75}    % 1

\definecolor{GnBuA}{RGB}{247,252,240} % 0
\definecolor{GnBuB}{RGB}{224,243,219} % 0.125
\definecolor{GnBuC}{RGB}{204,235,197} % 0.25
\definecolor{GnBuD}{RGB}{168,221,181} % 0.375
\definecolor{GnBuE}{RGB}{123,204,196} % 0.5
\definecolor{GnBuF}{RGB}{78,179,211}  % 0.625
\definecolor{GnBuG}{RGB}{43,140,190}  % 0.75
\definecolor{GnBuH}{RGB}{8,104,172}   % 0.875
\definecolor{GnBuI}{RGB}{8,64,129}    % 1.0

\definecolor{BuGnYlA}{RGB}{8,29,88} % 0
\definecolor{BuGnYlB}{RGB}{37,52,148} % 0.125
\definecolor{BuGnYlC}{RGB}{34,91,168} % 0.25
\definecolor{BuGnYlD}{RGB}{29,145,192} % 0.375
\definecolor{BuGnYlE}{RGB}{65,182,196} % 0.5
\definecolor{BuGnYlF}{RGB}{127,205,187}  % 0.625
\definecolor{BuGnYlG}{RGB}{199,233,180}  % 0.75
\definecolor{BuGnYlH}{RGB}{237,248,177}   % 0.875
\definecolor{BuGnYlI}{RGB}{255,255,217}    % 1.0

\definecolor{OrRdA}{RGB}{255,247,236} % 0
\definecolor{OrRdB}{RGB}{254,232,200} % 0.125
\definecolor{OrRdC}{RGB}{253,212,158} % 0.25
\definecolor{OrRdD}{RGB}{253,187,132} % 0.375
\definecolor{OrRdE}{RGB}{252,141,89} % 0.5
\definecolor{OrRdF}{RGB}{239,101,72}  % 0.625
\definecolor{OrRdG}{RGB}{215,48,31}  % 0.75
\definecolor{OrRdH}{RGB}{179,0,0}   % 0.875
\definecolor{OrRdI}{RGB}{127,0,0}    % 1.0

\definecolor{hotA}{RGB}{0,0,255}    % 0
\definecolor{hotB}{RGB}{0,255,255}  % 0.25
\definecolor{hotC}{RGB}{0,255,0}    % 0.5
\definecolor{hotD}{RGB}{255,255,0}  % 0.75
\definecolor{hotE}{RGB}{255,0,0}    % 1.0

\definecolor{uiucA}{RGB}{19,41,75}    % 0
\definecolor{uiucB}{RGB}{144,174,194} % 0.2
\definecolor{uiucC}{RGB}{228,243,250} % 0.4
\definecolor{uiucD}{RGB}{255,250,243} % 0.6
\definecolor{uiucE}{RGB}{255,193,172} % 0.8
\definecolor{uiucF}{RGB}{232,74,39}   % 1.0

\definecolor{MyBuGnA}{RGB}{37,91,207}    % 0
\definecolor{MyBuGnB}{RGB}{176,182,251}  % 0.2
\definecolor{MyBuGnC}{RGB}{246,239,255}  % 0.4
\definecolor{MyBuGnD}{RGB}{246,255,239}  % 0.6
\definecolor{MyBuGnE}{RGB}{176,251,182}  % 0.8
\definecolor{MyBuGnF}{RGB}{37,207,91}    % 1

\definecolor{MyBuRdA}{RGB}{37,91,207}    % 0
\definecolor{MyBuRdB}{RGB}{156,202,255}  % 0.2
\definecolor{MyBuRdC}{RGB}{232,252,255}  % 0.4
\definecolor{MyBuRdD}{RGB}{255,242,232}  % 0.6
\definecolor{MyBuRdE}{RGB}{255,170,156}  % 0.8
\definecolor{MyBuRdF}{RGB}{207,37,37}    % 1

\definecolor{MyViridisA}{RGB}{68,1,84}    % 0
\definecolor{MyViridisB}{RGB}{70,50,126}  % 0.25
\definecolor{MyViridisC}{RGB}{39,126,142}  % 0.5
\definecolor{MyViridisD}{RGB}{31,161,135}  % 0.75
\definecolor{MyViridisE}{RGB}{160,218,60}  % 1

\definecolor{xrayA}{RGB}{255,255,255}
\definecolor{xrayB}{RGB}{0,0,0}

\definecolor{MyHotA}{RGB}{0, 0, 255}    % 0
\definecolor{MyHotB}{RGB}{0, 96, 255}  % 0.25
\definecolor{MyHotC}{RGB}{0, 170, 255}  % 0.5
\definecolor{MyHotD}{RGB}{0, 223, 255}  % 0.75
\definecolor{MyHotE}{RGB}{0, 255, 255}  % 1
\definecolor{MyHotF}{RGB}{122, 255, 133}  % 1
\definecolor{MyHotG}{RGB}{255, 255, 0}  % 1
\definecolor{MyHotH}{RGB}{255, 223, 0}
\definecolor{MyHotI}{RGB}{255, 170, 0}
\definecolor{MyHotJ}{RGB}{255, 96, 0}
\definecolor{MyHotK}{RGB}{255, 0, 0}
\pgfplotsset{
colormap={MyHot}{
color(0)={MyHotA}
color(0.1)={MyHotB}
color(0.2)={MyHotC}
color(0.3)={MyHotD}
color(0.4)={MyHotE}
color(0.5)={MyHotF}
color(0.6)={MyHotG}
color(0.7)={MyHotH}
color(0.8)={MyHotI}
color(0.9)={MyHotJ}
color(1)={MyHotK}
}
}

\definecolor{MyJetA}{RGB}{37, 91, 207}    % 0
\definecolor{MyJetB}{RGB}{0, 177, 211}  % 0.25
\definecolor{MyJetC}{RGB}{37, 207, 91}  % 0.5
\definecolor{MyJetD}{RGB}{253, 180, 0}  % 0.75
\definecolor{MyJetE}{RGB}{253, 37, 37}  % 1
\pgfplotsset{
colormap={MyJet}{
color(0)={MyJetA}
color(0.25)={MyJetB}
color(0.5)={MyJetC}
color(0.75)={MyJetD}
color(1)={MyJetE}
}
}

\definecolor{VortA}{RGB}{37, 91, 207}    % 0
\definecolor{VortB}{RGB}{0, 177, 211}  % 0.25
\definecolor{VortC}{RGB}{37, 207, 91}  % 0.5
\definecolor{VortD}{RGB}{253, 180, 0}  % 0.75
\definecolor{VortE}{RGB}{253, 37, 37}  % 1
\pgfplotsset{
colormap={MyJet}{
color(0)={MyJetA}
color(0.25)={MyJetB}
color(0.5)={MyJetC}
color(0.75)={MyJetD}
color(1)={MyJetE}
}
}

\definecolor{MySpectralA}{RGB}{94, 79, 162}     % 0
\definecolor{MySpectralB}{RGB}{75, 126, 166}    % 0.2
\definecolor{MySpectralC}{RGB}{129, 193, 166}   % 0.4
\definecolor{MySpectralD}{RGB}{213, 238, 158}   % 0.6
\definecolor{MySpectralE}{RGB}{255, 203, 129}   % 0.8
\definecolor{MySpectralF}{RGB}{158, 1, 66}      % 1
\pgfplotsset{
colormap={MySpectral}{
color(0)={MySpectralA}
color(0.2)={MySpectralB}
color(0.4)={MySpectralC}
color(0.6)={MySpectralD}
color(0.8)={MySpectralE}
color(1)={MySpectralF}
}
}

\pgfplotsset{
colormap={Spectral}{
color(0)={SpectralA}
color(0.1)={SpectralB}
color(0.2)={SpectralC}
color(0.3)={SpectralD}
color(0.4)={SpectralE}
color(0.5)={SpectralF}
color(0.6)={SpectralG}
color(0.7)={SpectralH}
color(0.8)={SpectralI}
color(0.9)={SpectralJ}
color(1)={SpectralK}
},      
colormap={SpectralInverse}{
color(0)={SpectralK}
color(0.1)={SpectralJ}
color(0.2)={SpectralI}
color(0.3)={SpectralH}
color(0.4)={SpectralG}
color(0.5)={SpectralF}
color(0.6)={SpectralE}
color(0.7)={SpectralD}
color(0.8)={SpectralC}
color(0.9)={SpectralB}
color(1)={SpectralA}
},
colormap={GnBu}{
color(0)={GnBuA}
color(0.125)={GnBuB}
color(0.250)={GnBuC}
color(0.375)={GnBuD}
color(0.500)={GnBuE}
color(0.625)={GnBuF}
color(0.750)={GnBuG}
color(0.875)={GnBuH}
color(1)={GnBuI}
},
colormap={BuGnYl}{
color(0)={BuGnYlA}
color(0.125)={BuGnYlB}
color(0.250)={BuGnYlC}
color(0.375)={BuGnYlD}
color(0.500)={BuGnYlE}
color(0.625)={BuGnYlF}
color(0.750)={BuGnYlG}
color(0.875)={BuGnYlH}
color(1)={BuGnYlI}
},
colormap={RdBu}{
color(0)={RdBuA}
color(0.1)={RdBuB}
color(0.2)={RdBuC}
color(0.3)={RdBuD}
color(0.4)={RdBuE}
color(0.5)={RdBuF}
color(0.6)={RdBuG}
color(0.7)={RdBuH}
color(0.8)={RdBuI}
color(0.9)={RdBuJ}
color(1)={RdBuK}
},
colormap={BuRd}{
color(0)={RdBuK}
color(0.1)={RdBuJ}
color(0.2)={RdBuI}
color(0.3)={RdBuH}
color(0.4)={RdBuG}
color(0.5)={RdBuF}
color(0.6)={RdBuE}
color(0.7)={RdBuD}
color(0.8)={RdBuC}
color(0.9)={RdBuB}
color(1)={RdBuA}
},
colormap={RdYlBu}{
color(0)={RdYlBuA}
color(0.1)={RdYlBuB}
color(0.2)={RdYlBuC}
color(0.3)={RdYlBuD}
color(0.4)={RdYlBuE}
color(0.5)={RdYlBuF}
color(0.6)={RdYlBuG}
color(0.7)={RdYlBuH}
color(0.8)={RdYlBuI}
color(0.9)={RdYlBuJ}
color(1)={RdYlBuK}
},
colormap={RdYlBuInverse}{
color(0)={RdYlBuK}
color(0.1)={RdYlBuJ}
color(0.2)={RdYlBuI}
color(0.3)={RdYlBuH}
color(0.4)={RdYlBuG}
color(0.5)={RdYlBuF}
color(0.6)={RdYlBuE}
color(0.7)={RdYlBuD}
color(0.8)={RdYlBuC}
color(0.9)={RdYlBuB}
color(1)={RdYlBuA}
},
colormap={RdGy}{
color(0)={RdGyA}
color(0.1)={RdGyB}
color(0.2)={RdGyC}
color(0.3)={RdGyD}
color(0.4)={RdGyE}
color(0.5)={RdGyF}
color(0.6)={RdGyG}
color(0.7)={RdGyH}
color(0.8)={RdGyI}
color(0.9)={RdGyJ}
color(1)={RdGyK}
},
colormap={PuOr}{
color(0)={PuOrA}
color(0.1)={PuOrB}
color(0.2)={PuOrC}
color(0.3)={PuOrD}
color(0.4)={PuOrE}
color(0.5)={PuOrF}
color(0.6)={PuOrG}
color(0.7)={PuOrH}
color(0.8)={PuOrI}
color(0.9)={PuOrJ}
color(1)={PuOrK}
},
colormap={OrPu}{
color(0)={PuOrK}
color(0.1)={PuOrJ}
color(0.2)={PuOrI}
color(0.3)={PuOrH}
color(0.4)={PuOrG}
color(0.5)={PuOrF}
color(0.6)={PuOrE}
color(0.7)={PuOrD}
color(0.8)={PuOrC}
color(0.9)={PuOrB}
color(1)={PuOrA}
},
colormap={OrRd}{
color(0)={OrRdA}
color(0.125)={OrRdB}
color(0.250)={OrRdC}
color(0.375)={OrRdD}
color(0.500)={OrRdE}
color(0.625)={OrRdF}
color(0.750)={OrRdG}
color(0.875)={OrRdH}
color(1)={OrRdI}
},
colormap={RdOr}{
color(0)={OrRdI}
color(0.125)={OrRdH}
color(0.250)={OrRdG}
color(0.375)={OrRdF}
color(0.500)={OrRdE}
color(0.625)={OrRdD}
color(0.750)={OrRdC}
color(0.875)={OrRdB}
color(1)={OrRdA}
},
colormap={Hot}{
color(0)={hotA}
color(0.25)={hotB}
color(0.50)={hotC}
color(0.75)={hotD}
color(1)={hotE}
},
%
colormap={MyBuGn}{
color(0)={MyBuGnA}
color(0.2)={MyBuGnB}
color(0.4)={MyBuGnC}
color(0.6)={MyBuGnD}
color(0.8)={MyBuGnE},
color(1)={MyBuGnF}
},
%
colormap={MyBuRd}{
color(0)={MyBuRdA}
color(0.2)={MyBuRdB}
color(0.4)={MyBuRdC}
color(0.6)={MyBuRdD}
color(0.8)={MyBuRdE},
color(1)={MyBuRdF}
},
colormap={uiuc}{
color(0)={uiucA}
color(0.2)={uiucB}
color(0.4)={uiucC}
color(0.6)={uiucD}
color(0.8)={uiucE}
color(1)={uiucF}
},
colormap={viridis}{
color(0)={MyViridisE}
color(0.25)={MyViridisD}
color(0.5)={MyViridisC}
color(0.75)={MyViridisB}
color(1)={MyViridisA}
},
colormap={xray}{
color(0)={xrayA},
color(1)={xrayB}
},
colormap={xrayInverse}{
color(0)={xrayB},
color(1)={xrayA}
}
}


%% \usepackage{listings}
%% \lstdefinestyle{mystyle}{
%% backgroundcolor=\color{RYB2!10},   
%%     commentstyle=\color{RYB3},
%%     keywordstyle=\color{RYB1},
%%     numberstyle=\tiny\color{RYB0},
%%     stringstyle=\color{RYB4},
%%     basicstyle=\ttfamily\footnotesize,
%%     breakatwhitespace=false,         
%%     breaklines=true,                 
%%     captionpos=b,                    
%%     keepspaces=true,                 
%%     numbers=left,                    
%%     numbersep=5pt,                  
%%     showspaces=false,                
%%     showstringspaces=false,
%%     showtabs=false,                  
%%     tabsize=2
%% }
%% \lstset{style=mystyle}

\definecolor{plasma0}{RGB}{12, 7, 134}
\definecolor{plasma1}{RGB}{16, 7, 135}
\definecolor{plasma2}{RGB}{19, 6, 137}
\definecolor{plasma3}{RGB}{21, 6, 138}
\definecolor{plasma4}{RGB}{24, 6, 139}
\definecolor{plasma5}{RGB}{27, 6, 140}
\definecolor{plasma6}{RGB}{29, 6, 141}
\definecolor{plasma7}{RGB}{31, 5, 142}
\definecolor{plasma8}{RGB}{33, 5, 143}
\definecolor{plasma9}{RGB}{35, 5, 144}
\definecolor{plasma10}{RGB}{37, 5, 145}
\definecolor{plasma11}{RGB}{39, 5, 146}
\definecolor{plasma12}{RGB}{41, 5, 147}
\definecolor{plasma13}{RGB}{43, 5, 148}
\definecolor{plasma14}{RGB}{45, 4, 148}
\definecolor{plasma15}{RGB}{47, 4, 149}
\definecolor{plasma16}{RGB}{49, 4, 150}
\definecolor{plasma17}{RGB}{51, 4, 151}
\definecolor{plasma18}{RGB}{52, 4, 152}
\definecolor{plasma19}{RGB}{54, 4, 152}
\definecolor{plasma20}{RGB}{56, 4, 153}
\definecolor{plasma21}{RGB}{58, 4, 154}
\definecolor{plasma22}{RGB}{59, 3, 154}
\definecolor{plasma23}{RGB}{61, 3, 155}
\definecolor{plasma24}{RGB}{63, 3, 156}
\definecolor{plasma25}{RGB}{64, 3, 156}
\definecolor{plasma26}{RGB}{66, 3, 157}
\definecolor{plasma27}{RGB}{68, 3, 158}
\definecolor{plasma28}{RGB}{69, 3, 158}
\definecolor{plasma29}{RGB}{71, 2, 159}
\definecolor{plasma30}{RGB}{73, 2, 159}
\definecolor{plasma31}{RGB}{74, 2, 160}
\definecolor{plasma32}{RGB}{76, 2, 161}
\definecolor{plasma33}{RGB}{78, 2, 161}
\definecolor{plasma34}{RGB}{79, 2, 162}
\definecolor{plasma35}{RGB}{81, 1, 162}
\definecolor{plasma36}{RGB}{82, 1, 163}
\definecolor{plasma37}{RGB}{84, 1, 163}
\definecolor{plasma38}{RGB}{86, 1, 163}
\definecolor{plasma39}{RGB}{87, 1, 164}
\definecolor{plasma40}{RGB}{89, 1, 164}
\definecolor{plasma41}{RGB}{90, 0, 165}
\definecolor{plasma42}{RGB}{92, 0, 165}
\definecolor{plasma43}{RGB}{94, 0, 165}
\definecolor{plasma44}{RGB}{95, 0, 166}
\definecolor{plasma45}{RGB}{97, 0, 166}
\definecolor{plasma46}{RGB}{98, 0, 166}
\definecolor{plasma47}{RGB}{100, 0, 167}
\definecolor{plasma48}{RGB}{101, 0, 167}
\definecolor{plasma49}{RGB}{103, 0, 167}
\definecolor{plasma50}{RGB}{104, 0, 167}
\definecolor{plasma51}{RGB}{106, 0, 167}
\definecolor{plasma52}{RGB}{108, 0, 168}
\definecolor{plasma53}{RGB}{109, 0, 168}
\definecolor{plasma54}{RGB}{111, 0, 168}
\definecolor{plasma55}{RGB}{112, 0, 168}
\definecolor{plasma56}{RGB}{114, 0, 168}
\definecolor{plasma57}{RGB}{115, 0, 168}
\definecolor{plasma58}{RGB}{117, 0, 168}
\definecolor{plasma59}{RGB}{118, 1, 168}
\definecolor{plasma60}{RGB}{120, 1, 168}
\definecolor{plasma61}{RGB}{121, 1, 168}
\definecolor{plasma62}{RGB}{123, 2, 168}
\definecolor{plasma63}{RGB}{124, 2, 167}
\definecolor{plasma64}{RGB}{126, 3, 167}
\definecolor{plasma65}{RGB}{127, 3, 167}
\definecolor{plasma66}{RGB}{129, 4, 167}
\definecolor{plasma67}{RGB}{130, 4, 167}
\definecolor{plasma68}{RGB}{132, 5, 166}
\definecolor{plasma69}{RGB}{133, 6, 166}
\definecolor{plasma70}{RGB}{134, 7, 166}
\definecolor{plasma71}{RGB}{136, 7, 165}
\definecolor{plasma72}{RGB}{137, 8, 165}
\definecolor{plasma73}{RGB}{139, 9, 164}
\definecolor{plasma74}{RGB}{140, 10, 164}
\definecolor{plasma75}{RGB}{142, 12, 164}
\definecolor{plasma76}{RGB}{143, 13, 163}
\definecolor{plasma77}{RGB}{144, 14, 163}
\definecolor{plasma78}{RGB}{146, 15, 162}
\definecolor{plasma79}{RGB}{147, 16, 161}
\definecolor{plasma80}{RGB}{149, 17, 161}
\definecolor{plasma81}{RGB}{150, 18, 160}
\definecolor{plasma82}{RGB}{151, 19, 160}
\definecolor{plasma83}{RGB}{153, 20, 159}
\definecolor{plasma84}{RGB}{154, 21, 158}
\definecolor{plasma85}{RGB}{155, 23, 158}
\definecolor{plasma86}{RGB}{157, 24, 157}
\definecolor{plasma87}{RGB}{158, 25, 156}
\definecolor{plasma88}{RGB}{159, 26, 155}
\definecolor{plasma89}{RGB}{160, 27, 155}
\definecolor{plasma90}{RGB}{162, 28, 154}
\definecolor{plasma91}{RGB}{163, 29, 153}
\definecolor{plasma92}{RGB}{164, 30, 152}
\definecolor{plasma93}{RGB}{165, 31, 151}
\definecolor{plasma94}{RGB}{167, 33, 151}
\definecolor{plasma95}{RGB}{168, 34, 150}
\definecolor{plasma96}{RGB}{169, 35, 149}
\definecolor{plasma97}{RGB}{170, 36, 148}
\definecolor{plasma98}{RGB}{172, 37, 147}
\definecolor{plasma99}{RGB}{173, 38, 146}
\definecolor{plasma100}{RGB}{174, 39, 145}
\definecolor{plasma101}{RGB}{175, 40, 144}
\definecolor{plasma102}{RGB}{176, 42, 143}
\definecolor{plasma103}{RGB}{177, 43, 143}
\definecolor{plasma104}{RGB}{178, 44, 142}
\definecolor{plasma105}{RGB}{180, 45, 141}
\definecolor{plasma106}{RGB}{181, 46, 140}
\definecolor{plasma107}{RGB}{182, 47, 139}
\definecolor{plasma108}{RGB}{183, 48, 138}
\definecolor{plasma109}{RGB}{184, 50, 137}
\definecolor{plasma110}{RGB}{185, 51, 136}
\definecolor{plasma111}{RGB}{186, 52, 135}
\definecolor{plasma112}{RGB}{187, 53, 134}
\definecolor{plasma113}{RGB}{188, 54, 133}
\definecolor{plasma114}{RGB}{189, 55, 132}
\definecolor{plasma115}{RGB}{190, 56, 131}
\definecolor{plasma116}{RGB}{191, 57, 130}
\definecolor{plasma117}{RGB}{192, 59, 129}
\definecolor{plasma118}{RGB}{193, 60, 128}
\definecolor{plasma119}{RGB}{194, 61, 128}
\definecolor{plasma120}{RGB}{195, 62, 127}
\definecolor{plasma121}{RGB}{196, 63, 126}
\definecolor{plasma122}{RGB}{197, 64, 125}
\definecolor{plasma123}{RGB}{198, 65, 124}
\definecolor{plasma124}{RGB}{199, 66, 123}
\definecolor{plasma125}{RGB}{200, 68, 122}
\definecolor{plasma126}{RGB}{201, 69, 121}
\definecolor{plasma127}{RGB}{202, 70, 120}
\definecolor{plasma128}{RGB}{203, 71, 119}
\definecolor{plasma129}{RGB}{204, 72, 118}
\definecolor{plasma130}{RGB}{205, 73, 117}
\definecolor{plasma131}{RGB}{206, 74, 117}
\definecolor{plasma132}{RGB}{207, 75, 116}
\definecolor{plasma133}{RGB}{208, 77, 115}
\definecolor{plasma134}{RGB}{209, 78, 114}
\definecolor{plasma135}{RGB}{209, 79, 113}
\definecolor{plasma136}{RGB}{210, 80, 112}
\definecolor{plasma137}{RGB}{211, 81, 111}
\definecolor{plasma138}{RGB}{212, 82, 110}
\definecolor{plasma139}{RGB}{213, 83, 109}
\definecolor{plasma140}{RGB}{214, 85, 109}
\definecolor{plasma141}{RGB}{215, 86, 108}
\definecolor{plasma142}{RGB}{215, 87, 107}
\definecolor{plasma143}{RGB}{216, 88, 106}
\definecolor{plasma144}{RGB}{217, 89, 105}
\definecolor{plasma145}{RGB}{218, 90, 104}
\definecolor{plasma146}{RGB}{219, 91, 103}
\definecolor{plasma147}{RGB}{220, 93, 102}
\definecolor{plasma148}{RGB}{220, 94, 102}
\definecolor{plasma149}{RGB}{221, 95, 101}
\definecolor{plasma150}{RGB}{222, 96, 100}
\definecolor{plasma151}{RGB}{223, 97, 99}
\definecolor{plasma152}{RGB}{223, 98, 98}
\definecolor{plasma153}{RGB}{224, 100, 97}
\definecolor{plasma154}{RGB}{225, 101, 96}
\definecolor{plasma155}{RGB}{226, 102, 96}
\definecolor{plasma156}{RGB}{227, 103, 95}
\definecolor{plasma157}{RGB}{227, 104, 94}
\definecolor{plasma158}{RGB}{228, 106, 93}
\definecolor{plasma159}{RGB}{229, 107, 92}
\definecolor{plasma160}{RGB}{229, 108, 91}
\definecolor{plasma161}{RGB}{230, 109, 90}
\definecolor{plasma162}{RGB}{231, 110, 90}
\definecolor{plasma163}{RGB}{232, 112, 89}
\definecolor{plasma164}{RGB}{232, 113, 88}
\definecolor{plasma165}{RGB}{233, 114, 87}
\definecolor{plasma166}{RGB}{234, 115, 86}
\definecolor{plasma167}{RGB}{234, 116, 85}
\definecolor{plasma168}{RGB}{235, 118, 84}
\definecolor{plasma169}{RGB}{236, 119, 84}
\definecolor{plasma170}{RGB}{236, 120, 83}
\definecolor{plasma171}{RGB}{237, 121, 82}
\definecolor{plasma172}{RGB}{237, 123, 81}
\definecolor{plasma173}{RGB}{238, 124, 80}
\definecolor{plasma174}{RGB}{239, 125, 79}
\definecolor{plasma175}{RGB}{239, 126, 78}
\definecolor{plasma176}{RGB}{240, 128, 77}
\definecolor{plasma177}{RGB}{240, 129, 77}
\definecolor{plasma178}{RGB}{241, 130, 76}
\definecolor{plasma179}{RGB}{242, 132, 75}
\definecolor{plasma180}{RGB}{242, 133, 74}
\definecolor{plasma181}{RGB}{243, 134, 73}
\definecolor{plasma182}{RGB}{243, 135, 72}
\definecolor{plasma183}{RGB}{244, 137, 71}
\definecolor{plasma184}{RGB}{244, 138, 71}
\definecolor{plasma185}{RGB}{245, 139, 70}
\definecolor{plasma186}{RGB}{245, 141, 69}
\definecolor{plasma187}{RGB}{246, 142, 68}
\definecolor{plasma188}{RGB}{246, 143, 67}
\definecolor{plasma189}{RGB}{246, 145, 66}
\definecolor{plasma190}{RGB}{247, 146, 65}
\definecolor{plasma191}{RGB}{247, 147, 65}
\definecolor{plasma192}{RGB}{248, 149, 64}
\definecolor{plasma193}{RGB}{248, 150, 63}
\definecolor{plasma194}{RGB}{248, 152, 62}
\definecolor{plasma195}{RGB}{249, 153, 61}
\definecolor{plasma196}{RGB}{249, 154, 60}
\definecolor{plasma197}{RGB}{250, 156, 59}
\definecolor{plasma198}{RGB}{250, 157, 58}
\definecolor{plasma199}{RGB}{250, 159, 58}
\definecolor{plasma200}{RGB}{250, 160, 57}
\definecolor{plasma201}{RGB}{251, 162, 56}
\definecolor{plasma202}{RGB}{251, 163, 55}
\definecolor{plasma203}{RGB}{251, 164, 54}
\definecolor{plasma204}{RGB}{252, 166, 53}
\definecolor{plasma205}{RGB}{252, 167, 53}
\definecolor{plasma206}{RGB}{252, 169, 52}
\definecolor{plasma207}{RGB}{252, 170, 51}
\definecolor{plasma208}{RGB}{252, 172, 50}
\definecolor{plasma209}{RGB}{252, 173, 49}
\definecolor{plasma210}{RGB}{253, 175, 49}
\definecolor{plasma211}{RGB}{253, 176, 48}
\definecolor{plasma212}{RGB}{253, 178, 47}
\definecolor{plasma213}{RGB}{253, 179, 46}
\definecolor{plasma214}{RGB}{253, 181, 45}
\definecolor{plasma215}{RGB}{253, 182, 45}
\definecolor{plasma216}{RGB}{253, 184, 44}
\definecolor{plasma217}{RGB}{253, 185, 43}
\definecolor{plasma218}{RGB}{253, 187, 43}
\definecolor{plasma219}{RGB}{253, 188, 42}
\definecolor{plasma220}{RGB}{253, 190, 41}
\definecolor{plasma221}{RGB}{253, 192, 41}
\definecolor{plasma222}{RGB}{253, 193, 40}
\definecolor{plasma223}{RGB}{253, 195, 40}
\definecolor{plasma224}{RGB}{253, 196, 39}
\definecolor{plasma225}{RGB}{253, 198, 38}
\definecolor{plasma226}{RGB}{252, 199, 38}
\definecolor{plasma227}{RGB}{252, 201, 38}
\definecolor{plasma228}{RGB}{252, 203, 37}
\definecolor{plasma229}{RGB}{252, 204, 37}
\definecolor{plasma230}{RGB}{252, 206, 37}
\definecolor{plasma231}{RGB}{251, 208, 36}
\definecolor{plasma232}{RGB}{251, 209, 36}
\definecolor{plasma233}{RGB}{251, 211, 36}
\definecolor{plasma234}{RGB}{250, 213, 36}
\definecolor{plasma235}{RGB}{250, 214, 36}
\definecolor{plasma236}{RGB}{250, 216, 36}
\definecolor{plasma237}{RGB}{249, 217, 36}
\definecolor{plasma238}{RGB}{249, 219, 36}
\definecolor{plasma239}{RGB}{248, 221, 36}
\definecolor{plasma240}{RGB}{248, 223, 36}
\definecolor{plasma241}{RGB}{247, 224, 36}
\definecolor{plasma242}{RGB}{247, 226, 37}
\definecolor{plasma243}{RGB}{246, 228, 37}
\definecolor{plasma244}{RGB}{246, 229, 37}
\definecolor{plasma245}{RGB}{245, 231, 38}
\definecolor{plasma246}{RGB}{245, 233, 38}
\definecolor{plasma247}{RGB}{244, 234, 38}
\definecolor{plasma248}{RGB}{243, 236, 38}
\definecolor{plasma249}{RGB}{243, 238, 38}
\definecolor{plasma250}{RGB}{242, 240, 38}
\definecolor{plasma251}{RGB}{242, 241, 38}
\definecolor{plasma252}{RGB}{241, 243, 38}
\definecolor{plasma253}{RGB}{240, 245, 37}
\definecolor{plasma254}{RGB}{240, 246, 35}
\definecolor{plasma255}{RGB}{239, 248, 33}
\pgfplotsset{
colormap={plasma}{
color(0)={plasma0}
color(0.003921569)={plasma1}
color(0.007843138)={plasma2}
color(0.01176471)={plasma3}
color(0.01568628)={plasma4}
color(0.01960784)={plasma5}
color(0.02352941)={plasma6}
color(0.02745098)={plasma7}
color(0.03137255)={plasma8}
color(0.03529412)={plasma9}
color(0.03921569)={plasma10}
color(0.04313726)={plasma11}
color(0.04705882)={plasma12}
color(0.05098039)={plasma13}
color(0.05490196)={plasma14}
color(0.05882353)={plasma15}
color(0.0627451)={plasma16}
color(0.06666667)={plasma17}
color(0.07058824)={plasma18}
color(0.07450981)={plasma19}
color(0.07843138)={plasma20}
color(0.08235294)={plasma21}
color(0.08627451)={plasma22}
color(0.09019608)={plasma23}
color(0.09411765)={plasma24}
color(0.09803922)={plasma25}
color(0.1019608)={plasma26}
color(0.1058824)={plasma27}
color(0.1098039)={plasma28}
color(0.1137255)={plasma29}
color(0.1176471)={plasma30}
color(0.1215686)={plasma31}
color(0.1254902)={plasma32}
color(0.1294118)={plasma33}
color(0.1333333)={plasma34}
color(0.1372549)={plasma35}
color(0.1411765)={plasma36}
color(0.145098)={plasma37}
color(0.1490196)={plasma38}
color(0.1529412)={plasma39}
color(0.1568628)={plasma40}
color(0.1607843)={plasma41}
color(0.1647059)={plasma42}
color(0.1686275)={plasma43}
color(0.172549)={plasma44}
color(0.1764706)={plasma45}
color(0.1803922)={plasma46}
color(0.1843137)={plasma47}
color(0.1882353)={plasma48}
color(0.1921569)={plasma49}
color(0.1960784)={plasma50}
color(0.2)={plasma51}
color(0.2039216)={plasma52}
color(0.2078431)={plasma53}
color(0.2117647)={plasma54}
color(0.2156863)={plasma55}
color(0.2196078)={plasma56}
color(0.2235294)={plasma57}
color(0.227451)={plasma58}
color(0.2313726)={plasma59}
color(0.2352941)={plasma60}
color(0.2392157)={plasma61}
color(0.2431373)={plasma62}
color(0.2470588)={plasma63}
color(0.2509804)={plasma64}
color(0.254902)={plasma65}
color(0.2588235)={plasma66}
color(0.2627451)={plasma67}
color(0.2666667)={plasma68}
color(0.2705882)={plasma69}
color(0.2745098)={plasma70}
color(0.2784314)={plasma71}
color(0.282353)={plasma72}
color(0.2862745)={plasma73}
color(0.2901961)={plasma74}
color(0.2941177)={plasma75}
color(0.2980392)={plasma76}
color(0.3019608)={plasma77}
color(0.3058824)={plasma78}
color(0.3098039)={plasma79}
color(0.3137255)={plasma80}
color(0.3176471)={plasma81}
color(0.3215686)={plasma82}
color(0.3254902)={plasma83}
color(0.3294118)={plasma84}
color(0.3333333)={plasma85}
color(0.3372549)={plasma86}
color(0.3411765)={plasma87}
color(0.345098)={plasma88}
color(0.3490196)={plasma89}
color(0.3529412)={plasma90}
color(0.3568628)={plasma91}
color(0.3607843)={plasma92}
color(0.3647059)={plasma93}
color(0.3686275)={plasma94}
color(0.372549)={plasma95}
color(0.3764706)={plasma96}
color(0.3803922)={plasma97}
color(0.3843137)={plasma98}
color(0.3882353)={plasma99}
color(0.3921569)={plasma100}
color(0.3960784)={plasma101}
color(0.4)={plasma102}
color(0.4039216)={plasma103}
color(0.4078431)={plasma104}
color(0.4117647)={plasma105}
color(0.4156863)={plasma106}
color(0.4196078)={plasma107}
color(0.4235294)={plasma108}
color(0.427451)={plasma109}
color(0.4313726)={plasma110}
color(0.4352941)={plasma111}
color(0.4392157)={plasma112}
color(0.4431373)={plasma113}
color(0.4470588)={plasma114}
color(0.4509804)={plasma115}
color(0.454902)={plasma116}
color(0.4588235)={plasma117}
color(0.4627451)={plasma118}
color(0.4666667)={plasma119}
color(0.4705882)={plasma120}
color(0.4745098)={plasma121}
color(0.4784314)={plasma122}
color(0.4823529)={plasma123}
color(0.4862745)={plasma124}
color(0.4901961)={plasma125}
color(0.4941176)={plasma126}
color(0.4980392)={plasma127}
color(0.5019608)={plasma128}
color(0.5058824)={plasma129}
color(0.509804)={plasma130}
color(0.5137255)={plasma131}
color(0.5176471)={plasma132}
color(0.5215687)={plasma133}
color(0.5254902)={plasma134}
color(0.5294118)={plasma135}
color(0.5333334)={plasma136}
color(0.5372549)={plasma137}
color(0.5411765)={plasma138}
color(0.5450981)={plasma139}
color(0.5490196)={plasma140}
color(0.5529412)={plasma141}
color(0.5568628)={plasma142}
color(0.5607843)={plasma143}
color(0.5647059)={plasma144}
color(0.5686275)={plasma145}
color(0.572549)={plasma146}
color(0.5764706)={plasma147}
color(0.5803922)={plasma148}
color(0.5843138)={plasma149}
color(0.5882353)={plasma150}
color(0.5921569)={plasma151}
color(0.5960785)={plasma152}
color(0.6)={plasma153}
color(0.6039216)={plasma154}
color(0.6078432)={plasma155}
color(0.6117647)={plasma156}
color(0.6156863)={plasma157}
color(0.6196079)={plasma158}
color(0.6235294)={plasma159}
color(0.627451)={plasma160}
color(0.6313726)={plasma161}
color(0.6352941)={plasma162}
color(0.6392157)={plasma163}
color(0.6431373)={plasma164}
color(0.6470588)={plasma165}
color(0.6509804)={plasma166}
color(0.654902)={plasma167}
color(0.6588235)={plasma168}
color(0.6627451)={plasma169}
color(0.6666667)={plasma170}
color(0.6705883)={plasma171}
color(0.6745098)={plasma172}
color(0.6784314)={plasma173}
color(0.682353)={plasma174}
color(0.6862745)={plasma175}
color(0.6901961)={plasma176}
color(0.6941177)={plasma177}
color(0.6980392)={plasma178}
color(0.7019608)={plasma179}
color(0.7058824)={plasma180}
color(0.7098039)={plasma181}
color(0.7137255)={plasma182}
color(0.7176471)={plasma183}
color(0.7215686)={plasma184}
color(0.7254902)={plasma185}
color(0.7294118)={plasma186}
color(0.7333333)={plasma187}
color(0.7372549)={plasma188}
color(0.7411765)={plasma189}
color(0.7450981)={plasma190}
color(0.7490196)={plasma191}
color(0.7529412)={plasma192}
color(0.7568628)={plasma193}
color(0.7607843)={plasma194}
color(0.7647059)={plasma195}
color(0.7686275)={plasma196}
color(0.772549)={plasma197}
color(0.7764706)={plasma198}
color(0.7803922)={plasma199}
color(0.7843137)={plasma200}
color(0.7882353)={plasma201}
color(0.7921569)={plasma202}
color(0.7960784)={plasma203}
color(0.8)={plasma204}
color(0.8039216)={plasma205}
color(0.8078431)={plasma206}
color(0.8117647)={plasma207}
color(0.8156863)={plasma208}
color(0.8196079)={plasma209}
color(0.8235294)={plasma210}
color(0.827451)={plasma211}
color(0.8313726)={plasma212}
color(0.8352941)={plasma213}
color(0.8392157)={plasma214}
color(0.8431373)={plasma215}
color(0.8470588)={plasma216}
color(0.8509804)={plasma217}
color(0.854902)={plasma218}
color(0.8588235)={plasma219}
color(0.8627451)={plasma220}
color(0.8666667)={plasma221}
color(0.8705882)={plasma222}
color(0.8745098)={plasma223}
color(0.8784314)={plasma224}
color(0.8823529)={plasma225}
color(0.8862745)={plasma226}
color(0.8901961)={plasma227}
color(0.8941177)={plasma228}
color(0.8980392)={plasma229}
color(0.9019608)={plasma230}
color(0.9058824)={plasma231}
color(0.9098039)={plasma232}
color(0.9137255)={plasma233}
color(0.9176471)={plasma234}
color(0.9215686)={plasma235}
color(0.9254902)={plasma236}
color(0.9294118)={plasma237}
color(0.9333333)={plasma238}
color(0.9372549)={plasma239}
color(0.9411765)={plasma240}
color(0.945098)={plasma241}
color(0.9490196)={plasma242}
color(0.9529412)={plasma243}
color(0.9568627)={plasma244}
color(0.9607843)={plasma245}
color(0.9647059)={plasma246}
color(0.9686275)={plasma247}
color(0.972549)={plasma248}
color(0.9764706)={plasma249}
color(0.9803922)={plasma250}
color(0.9843137)={plasma251}
color(0.9882353)={plasma252}
color(0.9921569)={plasma253}
color(0.9960784)={plasma254}
color(1)={plasma255}
}
}

\definecolor{inferno0}{RGB}{0, 0, 3}
\definecolor{inferno1}{RGB}{0, 0, 4}
\definecolor{inferno2}{RGB}{0, 0, 6}
\definecolor{inferno3}{RGB}{1, 0, 7}
\definecolor{inferno4}{RGB}{1, 1, 9}
\definecolor{inferno5}{RGB}{1, 1, 11}
\definecolor{inferno6}{RGB}{2, 1, 14}
\definecolor{inferno7}{RGB}{2, 2, 16}
\definecolor{inferno8}{RGB}{3, 2, 18}
\definecolor{inferno9}{RGB}{4, 3, 20}
\definecolor{inferno10}{RGB}{4, 3, 22}
\definecolor{inferno11}{RGB}{5, 4, 24}
\definecolor{inferno12}{RGB}{6, 4, 27}
\definecolor{inferno13}{RGB}{7, 5, 29}
\definecolor{inferno14}{RGB}{8, 6, 31}
\definecolor{inferno15}{RGB}{9, 6, 33}
\definecolor{inferno16}{RGB}{10, 7, 35}
\definecolor{inferno17}{RGB}{11, 7, 38}
\definecolor{inferno18}{RGB}{13, 8, 40}
\definecolor{inferno19}{RGB}{14, 8, 42}
\definecolor{inferno20}{RGB}{15, 9, 45}
\definecolor{inferno21}{RGB}{16, 9, 47}
\definecolor{inferno22}{RGB}{18, 10, 50}
\definecolor{inferno23}{RGB}{19, 10, 52}
\definecolor{inferno24}{RGB}{20, 11, 54}
\definecolor{inferno25}{RGB}{22, 11, 57}
\definecolor{inferno26}{RGB}{23, 11, 59}
\definecolor{inferno27}{RGB}{25, 11, 62}
\definecolor{inferno28}{RGB}{26, 11, 64}
\definecolor{inferno29}{RGB}{28, 12, 67}
\definecolor{inferno30}{RGB}{29, 12, 69}
\definecolor{inferno31}{RGB}{31, 12, 71}
\definecolor{inferno32}{RGB}{32, 12, 74}
\definecolor{inferno33}{RGB}{34, 11, 76}
\definecolor{inferno34}{RGB}{36, 11, 78}
\definecolor{inferno35}{RGB}{38, 11, 80}
\definecolor{inferno36}{RGB}{39, 11, 82}
\definecolor{inferno37}{RGB}{41, 11, 84}
\definecolor{inferno38}{RGB}{43, 10, 86}
\definecolor{inferno39}{RGB}{45, 10, 88}
\definecolor{inferno40}{RGB}{46, 10, 90}
\definecolor{inferno41}{RGB}{48, 10, 92}
\definecolor{inferno42}{RGB}{50, 9, 93}
\definecolor{inferno43}{RGB}{52, 9, 95}
\definecolor{inferno44}{RGB}{53, 9, 96}
\definecolor{inferno45}{RGB}{55, 9, 97}
\definecolor{inferno46}{RGB}{57, 9, 98}
\definecolor{inferno47}{RGB}{59, 9, 100}
\definecolor{inferno48}{RGB}{60, 9, 101}
\definecolor{inferno49}{RGB}{62, 9, 102}
\definecolor{inferno50}{RGB}{64, 9, 102}
\definecolor{inferno51}{RGB}{65, 9, 103}
\definecolor{inferno52}{RGB}{67, 10, 104}
\definecolor{inferno53}{RGB}{69, 10, 105}
\definecolor{inferno54}{RGB}{70, 10, 105}
\definecolor{inferno55}{RGB}{72, 11, 106}
\definecolor{inferno56}{RGB}{74, 11, 106}
\definecolor{inferno57}{RGB}{75, 12, 107}
\definecolor{inferno58}{RGB}{77, 12, 107}
\definecolor{inferno59}{RGB}{79, 13, 108}
\definecolor{inferno60}{RGB}{80, 13, 108}
\definecolor{inferno61}{RGB}{82, 14, 108}
\definecolor{inferno62}{RGB}{83, 14, 109}
\definecolor{inferno63}{RGB}{85, 15, 109}
\definecolor{inferno64}{RGB}{87, 15, 109}
\definecolor{inferno65}{RGB}{88, 16, 109}
\definecolor{inferno66}{RGB}{90, 17, 109}
\definecolor{inferno67}{RGB}{91, 17, 110}
\definecolor{inferno68}{RGB}{93, 18, 110}
\definecolor{inferno69}{RGB}{95, 18, 110}
\definecolor{inferno70}{RGB}{96, 19, 110}
\definecolor{inferno71}{RGB}{98, 20, 110}
\definecolor{inferno72}{RGB}{99, 20, 110}
\definecolor{inferno73}{RGB}{101, 21, 110}
\definecolor{inferno74}{RGB}{102, 21, 110}
\definecolor{inferno75}{RGB}{104, 22, 110}
\definecolor{inferno76}{RGB}{106, 23, 110}
\definecolor{inferno77}{RGB}{107, 23, 110}
\definecolor{inferno78}{RGB}{109, 24, 110}
\definecolor{inferno79}{RGB}{110, 24, 110}
\definecolor{inferno80}{RGB}{112, 25, 110}
\definecolor{inferno81}{RGB}{114, 25, 109}
\definecolor{inferno82}{RGB}{115, 26, 109}
\definecolor{inferno83}{RGB}{117, 27, 109}
\definecolor{inferno84}{RGB}{118, 27, 109}
\definecolor{inferno85}{RGB}{120, 28, 109}
\definecolor{inferno86}{RGB}{122, 28, 109}
\definecolor{inferno87}{RGB}{123, 29, 108}
\definecolor{inferno88}{RGB}{125, 29, 108}
\definecolor{inferno89}{RGB}{126, 30, 108}
\definecolor{inferno90}{RGB}{128, 31, 107}
\definecolor{inferno91}{RGB}{129, 31, 107}
\definecolor{inferno92}{RGB}{131, 32, 107}
\definecolor{inferno93}{RGB}{133, 32, 106}
\definecolor{inferno94}{RGB}{134, 33, 106}
\definecolor{inferno95}{RGB}{136, 33, 106}
\definecolor{inferno96}{RGB}{137, 34, 105}
\definecolor{inferno97}{RGB}{139, 34, 105}
\definecolor{inferno98}{RGB}{141, 35, 105}
\definecolor{inferno99}{RGB}{142, 36, 104}
\definecolor{inferno100}{RGB}{144, 36, 104}
\definecolor{inferno101}{RGB}{145, 37, 103}
\definecolor{inferno102}{RGB}{147, 37, 103}
\definecolor{inferno103}{RGB}{149, 38, 102}
\definecolor{inferno104}{RGB}{150, 38, 102}
\definecolor{inferno105}{RGB}{152, 39, 101}
\definecolor{inferno106}{RGB}{153, 40, 100}
\definecolor{inferno107}{RGB}{155, 40, 100}
\definecolor{inferno108}{RGB}{156, 41, 99}
\definecolor{inferno109}{RGB}{158, 41, 99}
\definecolor{inferno110}{RGB}{160, 42, 98}
\definecolor{inferno111}{RGB}{161, 43, 97}
\definecolor{inferno112}{RGB}{163, 43, 97}
\definecolor{inferno113}{RGB}{164, 44, 96}
\definecolor{inferno114}{RGB}{166, 44, 95}
\definecolor{inferno115}{RGB}{167, 45, 95}
\definecolor{inferno116}{RGB}{169, 46, 94}
\definecolor{inferno117}{RGB}{171, 46, 93}
\definecolor{inferno118}{RGB}{172, 47, 92}
\definecolor{inferno119}{RGB}{174, 48, 91}
\definecolor{inferno120}{RGB}{175, 49, 91}
\definecolor{inferno121}{RGB}{177, 49, 90}
\definecolor{inferno122}{RGB}{178, 50, 89}
\definecolor{inferno123}{RGB}{180, 51, 88}
\definecolor{inferno124}{RGB}{181, 51, 87}
\definecolor{inferno125}{RGB}{183, 52, 86}
\definecolor{inferno126}{RGB}{184, 53, 86}
\definecolor{inferno127}{RGB}{186, 54, 85}
\definecolor{inferno128}{RGB}{187, 55, 84}
\definecolor{inferno129}{RGB}{189, 55, 83}
\definecolor{inferno130}{RGB}{190, 56, 82}
\definecolor{inferno131}{RGB}{191, 57, 81}
\definecolor{inferno132}{RGB}{193, 58, 80}
\definecolor{inferno133}{RGB}{194, 59, 79}
\definecolor{inferno134}{RGB}{196, 60, 78}
\definecolor{inferno135}{RGB}{197, 61, 77}
\definecolor{inferno136}{RGB}{199, 62, 76}
\definecolor{inferno137}{RGB}{200, 62, 75}
\definecolor{inferno138}{RGB}{201, 63, 74}
\definecolor{inferno139}{RGB}{203, 64, 73}
\definecolor{inferno140}{RGB}{204, 65, 72}
\definecolor{inferno141}{RGB}{205, 66, 71}
\definecolor{inferno142}{RGB}{207, 68, 70}
\definecolor{inferno143}{RGB}{208, 69, 68}
\definecolor{inferno144}{RGB}{209, 70, 67}
\definecolor{inferno145}{RGB}{210, 71, 66}
\definecolor{inferno146}{RGB}{212, 72, 65}
\definecolor{inferno147}{RGB}{213, 73, 64}
\definecolor{inferno148}{RGB}{214, 74, 63}
\definecolor{inferno149}{RGB}{215, 75, 62}
\definecolor{inferno150}{RGB}{217, 77, 61}
\definecolor{inferno151}{RGB}{218, 78, 59}
\definecolor{inferno152}{RGB}{219, 79, 58}
\definecolor{inferno153}{RGB}{220, 80, 57}
\definecolor{inferno154}{RGB}{221, 82, 56}
\definecolor{inferno155}{RGB}{222, 83, 55}
\definecolor{inferno156}{RGB}{223, 84, 54}
\definecolor{inferno157}{RGB}{224, 86, 52}
\definecolor{inferno158}{RGB}{226, 87, 51}
\definecolor{inferno159}{RGB}{227, 88, 50}
\definecolor{inferno160}{RGB}{228, 90, 49}
\definecolor{inferno161}{RGB}{229, 91, 48}
\definecolor{inferno162}{RGB}{230, 92, 46}
\definecolor{inferno163}{RGB}{230, 94, 45}
\definecolor{inferno164}{RGB}{231, 95, 44}
\definecolor{inferno165}{RGB}{232, 97, 43}
\definecolor{inferno166}{RGB}{233, 98, 42}
\definecolor{inferno167}{RGB}{234, 100, 40}
\definecolor{inferno168}{RGB}{235, 101, 39}
\definecolor{inferno169}{RGB}{236, 103, 38}
\definecolor{inferno170}{RGB}{237, 104, 37}
\definecolor{inferno171}{RGB}{237, 106, 35}
\definecolor{inferno172}{RGB}{238, 108, 34}
\definecolor{inferno173}{RGB}{239, 109, 33}
\definecolor{inferno174}{RGB}{240, 111, 31}
\definecolor{inferno175}{RGB}{240, 112, 30}
\definecolor{inferno176}{RGB}{241, 114, 29}
\definecolor{inferno177}{RGB}{242, 116, 28}
\definecolor{inferno178}{RGB}{242, 117, 26}
\definecolor{inferno179}{RGB}{243, 119, 25}
\definecolor{inferno180}{RGB}{243, 121, 24}
\definecolor{inferno181}{RGB}{244, 122, 22}
\definecolor{inferno182}{RGB}{245, 124, 21}
\definecolor{inferno183}{RGB}{245, 126, 20}
\definecolor{inferno184}{RGB}{246, 128, 18}
\definecolor{inferno185}{RGB}{246, 129, 17}
\definecolor{inferno186}{RGB}{247, 131, 16}
\definecolor{inferno187}{RGB}{247, 133, 14}
\definecolor{inferno188}{RGB}{248, 135, 13}
\definecolor{inferno189}{RGB}{248, 136, 12}
\definecolor{inferno190}{RGB}{248, 138, 11}
\definecolor{inferno191}{RGB}{249, 140, 9}
\definecolor{inferno192}{RGB}{249, 142, 8}
\definecolor{inferno193}{RGB}{249, 144, 8}
\definecolor{inferno194}{RGB}{250, 145, 7}
\definecolor{inferno195}{RGB}{250, 147, 6}
\definecolor{inferno196}{RGB}{250, 149, 6}
\definecolor{inferno197}{RGB}{250, 151, 6}
\definecolor{inferno198}{RGB}{251, 153, 6}
\definecolor{inferno199}{RGB}{251, 155, 6}
\definecolor{inferno200}{RGB}{251, 157, 6}
\definecolor{inferno201}{RGB}{251, 158, 7}
\definecolor{inferno202}{RGB}{251, 160, 7}
\definecolor{inferno203}{RGB}{251, 162, 8}
\definecolor{inferno204}{RGB}{251, 164, 10}
\definecolor{inferno205}{RGB}{251, 166, 11}
\definecolor{inferno206}{RGB}{251, 168, 13}
\definecolor{inferno207}{RGB}{251, 170, 14}
\definecolor{inferno208}{RGB}{251, 172, 16}
\definecolor{inferno209}{RGB}{251, 174, 18}
\definecolor{inferno210}{RGB}{251, 176, 20}
\definecolor{inferno211}{RGB}{251, 177, 22}
\definecolor{inferno212}{RGB}{251, 179, 24}
\definecolor{inferno213}{RGB}{251, 181, 26}
\definecolor{inferno214}{RGB}{251, 183, 28}
\definecolor{inferno215}{RGB}{251, 185, 30}
\definecolor{inferno216}{RGB}{250, 187, 33}
\definecolor{inferno217}{RGB}{250, 189, 35}
\definecolor{inferno218}{RGB}{250, 191, 37}
\definecolor{inferno219}{RGB}{250, 193, 40}
\definecolor{inferno220}{RGB}{249, 195, 42}
\definecolor{inferno221}{RGB}{249, 197, 44}
\definecolor{inferno222}{RGB}{249, 199, 47}
\definecolor{inferno223}{RGB}{248, 201, 49}
\definecolor{inferno224}{RGB}{248, 203, 52}
\definecolor{inferno225}{RGB}{248, 205, 55}
\definecolor{inferno226}{RGB}{247, 207, 58}
\definecolor{inferno227}{RGB}{247, 209, 60}
\definecolor{inferno228}{RGB}{246, 211, 63}
\definecolor{inferno229}{RGB}{246, 213, 66}
\definecolor{inferno230}{RGB}{245, 215, 69}
\definecolor{inferno231}{RGB}{245, 217, 72}
\definecolor{inferno232}{RGB}{244, 219, 75}
\definecolor{inferno233}{RGB}{244, 220, 79}
\definecolor{inferno234}{RGB}{243, 222, 82}
\definecolor{inferno235}{RGB}{243, 224, 86}
\definecolor{inferno236}{RGB}{243, 226, 89}
\definecolor{inferno237}{RGB}{242, 228, 93}
\definecolor{inferno238}{RGB}{242, 230, 96}
\definecolor{inferno239}{RGB}{241, 232, 100}
\definecolor{inferno240}{RGB}{241, 233, 104}
\definecolor{inferno241}{RGB}{241, 235, 108}
\definecolor{inferno242}{RGB}{241, 237, 112}
\definecolor{inferno243}{RGB}{241, 238, 116}
\definecolor{inferno244}{RGB}{241, 240, 121}
\definecolor{inferno245}{RGB}{241, 242, 125}
\definecolor{inferno246}{RGB}{242, 243, 129}
\definecolor{inferno247}{RGB}{242, 244, 133}
\definecolor{inferno248}{RGB}{243, 246, 137}
\definecolor{inferno249}{RGB}{244, 247, 141}
\definecolor{inferno250}{RGB}{245, 248, 145}
\definecolor{inferno251}{RGB}{246, 250, 149}
\definecolor{inferno252}{RGB}{247, 251, 153}
\definecolor{inferno253}{RGB}{249, 252, 157}
\definecolor{inferno254}{RGB}{250, 253, 160}
\definecolor{inferno255}{RGB}{252, 254, 164}
\pgfplotsset{
colormap={inferno}{
color(0)={inferno0}
color(0.003921569)={inferno1}
color(0.007843138)={inferno2}
color(0.01176471)={inferno3}
color(0.01568628)={inferno4}
color(0.01960784)={inferno5}
color(0.02352941)={inferno6}
color(0.02745098)={inferno7}
color(0.03137255)={inferno8}
color(0.03529412)={inferno9}
color(0.03921569)={inferno10}
color(0.04313726)={inferno11}
color(0.04705882)={inferno12}
color(0.05098039)={inferno13}
color(0.05490196)={inferno14}
color(0.05882353)={inferno15}
color(0.0627451)={inferno16}
color(0.06666667)={inferno17}
color(0.07058824)={inferno18}
color(0.07450981)={inferno19}
color(0.07843138)={inferno20}
color(0.08235294)={inferno21}
color(0.08627451)={inferno22}
color(0.09019608)={inferno23}
color(0.09411765)={inferno24}
color(0.09803922)={inferno25}
color(0.1019608)={inferno26}
color(0.1058824)={inferno27}
color(0.1098039)={inferno28}
color(0.1137255)={inferno29}
color(0.1176471)={inferno30}
color(0.1215686)={inferno31}
color(0.1254902)={inferno32}
color(0.1294118)={inferno33}
color(0.1333333)={inferno34}
color(0.1372549)={inferno35}
color(0.1411765)={inferno36}
color(0.145098)={inferno37}
color(0.1490196)={inferno38}
color(0.1529412)={inferno39}
color(0.1568628)={inferno40}
color(0.1607843)={inferno41}
color(0.1647059)={inferno42}
color(0.1686275)={inferno43}
color(0.172549)={inferno44}
color(0.1764706)={inferno45}
color(0.1803922)={inferno46}
color(0.1843137)={inferno47}
color(0.1882353)={inferno48}
color(0.1921569)={inferno49}
color(0.1960784)={inferno50}
color(0.2)={inferno51}
color(0.2039216)={inferno52}
color(0.2078431)={inferno53}
color(0.2117647)={inferno54}
color(0.2156863)={inferno55}
color(0.2196078)={inferno56}
color(0.2235294)={inferno57}
color(0.227451)={inferno58}
color(0.2313726)={inferno59}
color(0.2352941)={inferno60}
color(0.2392157)={inferno61}
color(0.2431373)={inferno62}
color(0.2470588)={inferno63}
color(0.2509804)={inferno64}
color(0.254902)={inferno65}
color(0.2588235)={inferno66}
color(0.2627451)={inferno67}
color(0.2666667)={inferno68}
color(0.2705882)={inferno69}
color(0.2745098)={inferno70}
color(0.2784314)={inferno71}
color(0.282353)={inferno72}
color(0.2862745)={inferno73}
color(0.2901961)={inferno74}
color(0.2941177)={inferno75}
color(0.2980392)={inferno76}
color(0.3019608)={inferno77}
color(0.3058824)={inferno78}
color(0.3098039)={inferno79}
color(0.3137255)={inferno80}
color(0.3176471)={inferno81}
color(0.3215686)={inferno82}
color(0.3254902)={inferno83}
color(0.3294118)={inferno84}
color(0.3333333)={inferno85}
color(0.3372549)={inferno86}
color(0.3411765)={inferno87}
color(0.345098)={inferno88}
color(0.3490196)={inferno89}
color(0.3529412)={inferno90}
color(0.3568628)={inferno91}
color(0.3607843)={inferno92}
color(0.3647059)={inferno93}
color(0.3686275)={inferno94}
color(0.372549)={inferno95}
color(0.3764706)={inferno96}
color(0.3803922)={inferno97}
color(0.3843137)={inferno98}
color(0.3882353)={inferno99}
color(0.3921569)={inferno100}
color(0.3960784)={inferno101}
color(0.4)={inferno102}
color(0.4039216)={inferno103}
color(0.4078431)={inferno104}
color(0.4117647)={inferno105}
color(0.4156863)={inferno106}
color(0.4196078)={inferno107}
color(0.4235294)={inferno108}
color(0.427451)={inferno109}
color(0.4313726)={inferno110}
color(0.4352941)={inferno111}
color(0.4392157)={inferno112}
color(0.4431373)={inferno113}
color(0.4470588)={inferno114}
color(0.4509804)={inferno115}
color(0.454902)={inferno116}
color(0.4588235)={inferno117}
color(0.4627451)={inferno118}
color(0.4666667)={inferno119}
color(0.4705882)={inferno120}
color(0.4745098)={inferno121}
color(0.4784314)={inferno122}
color(0.4823529)={inferno123}
color(0.4862745)={inferno124}
color(0.4901961)={inferno125}
color(0.4941176)={inferno126}
color(0.4980392)={inferno127}
color(0.5019608)={inferno128}
color(0.5058824)={inferno129}
color(0.509804)={inferno130}
color(0.5137255)={inferno131}
color(0.5176471)={inferno132}
color(0.5215687)={inferno133}
color(0.5254902)={inferno134}
color(0.5294118)={inferno135}
color(0.5333334)={inferno136}
color(0.5372549)={inferno137}
color(0.5411765)={inferno138}
color(0.5450981)={inferno139}
color(0.5490196)={inferno140}
color(0.5529412)={inferno141}
color(0.5568628)={inferno142}
color(0.5607843)={inferno143}
color(0.5647059)={inferno144}
color(0.5686275)={inferno145}
color(0.572549)={inferno146}
color(0.5764706)={inferno147}
color(0.5803922)={inferno148}
color(0.5843138)={inferno149}
color(0.5882353)={inferno150}
color(0.5921569)={inferno151}
color(0.5960785)={inferno152}
color(0.6)={inferno153}
color(0.6039216)={inferno154}
color(0.6078432)={inferno155}
color(0.6117647)={inferno156}
color(0.6156863)={inferno157}
color(0.6196079)={inferno158}
color(0.6235294)={inferno159}
color(0.627451)={inferno160}
color(0.6313726)={inferno161}
color(0.6352941)={inferno162}
color(0.6392157)={inferno163}
color(0.6431373)={inferno164}
color(0.6470588)={inferno165}
color(0.6509804)={inferno166}
color(0.654902)={inferno167}
color(0.6588235)={inferno168}
color(0.6627451)={inferno169}
color(0.6666667)={inferno170}
color(0.6705883)={inferno171}
color(0.6745098)={inferno172}
color(0.6784314)={inferno173}
color(0.682353)={inferno174}
color(0.6862745)={inferno175}
color(0.6901961)={inferno176}
color(0.6941177)={inferno177}
color(0.6980392)={inferno178}
color(0.7019608)={inferno179}
color(0.7058824)={inferno180}
color(0.7098039)={inferno181}
color(0.7137255)={inferno182}
color(0.7176471)={inferno183}
color(0.7215686)={inferno184}
color(0.7254902)={inferno185}
color(0.7294118)={inferno186}
color(0.7333333)={inferno187}
color(0.7372549)={inferno188}
color(0.7411765)={inferno189}
color(0.7450981)={inferno190}
color(0.7490196)={inferno191}
color(0.7529412)={inferno192}
color(0.7568628)={inferno193}
color(0.7607843)={inferno194}
color(0.7647059)={inferno195}
color(0.7686275)={inferno196}
color(0.772549)={inferno197}
color(0.7764706)={inferno198}
color(0.7803922)={inferno199}
color(0.7843137)={inferno200}
color(0.7882353)={inferno201}
color(0.7921569)={inferno202}
color(0.7960784)={inferno203}
color(0.8)={inferno204}
color(0.8039216)={inferno205}
color(0.8078431)={inferno206}
color(0.8117647)={inferno207}
color(0.8156863)={inferno208}
color(0.8196079)={inferno209}
color(0.8235294)={inferno210}
color(0.827451)={inferno211}
color(0.8313726)={inferno212}
color(0.8352941)={inferno213}
color(0.8392157)={inferno214}
color(0.8431373)={inferno215}
color(0.8470588)={inferno216}
color(0.8509804)={inferno217}
color(0.854902)={inferno218}
color(0.8588235)={inferno219}
color(0.8627451)={inferno220}
color(0.8666667)={inferno221}
color(0.8705882)={inferno222}
color(0.8745098)={inferno223}
color(0.8784314)={inferno224}
color(0.8823529)={inferno225}
color(0.8862745)={inferno226}
color(0.8901961)={inferno227}
color(0.8941177)={inferno228}
color(0.8980392)={inferno229}
color(0.9019608)={inferno230}
color(0.9058824)={inferno231}
color(0.9098039)={inferno232}
color(0.9137255)={inferno233}
color(0.9176471)={inferno234}
color(0.9215686)={inferno235}
color(0.9254902)={inferno236}
color(0.9294118)={inferno237}
color(0.9333333)={inferno238}
color(0.9372549)={inferno239}
color(0.9411765)={inferno240}
color(0.945098)={inferno241}
color(0.9490196)={inferno242}
color(0.9529412)={inferno243}
color(0.9568627)={inferno244}
color(0.9607843)={inferno245}
color(0.9647059)={inferno246}
color(0.9686275)={inferno247}
color(0.972549)={inferno248}
color(0.9764706)={inferno249}
color(0.9803922)={inferno250}
color(0.9843137)={inferno251}
color(0.9882353)={inferno252}
color(0.9921569)={inferno253}
color(0.9960784)={inferno254}
color(1)={inferno255}
}
}

\definecolor{hot_desaturated0}{RGB}{71, 71, 219}
\definecolor{hot_desaturated1}{RGB}{0, 0, 91}
\definecolor{hot_desaturated2}{RGB}{0, 255, 255}
\definecolor{hot_desaturated3}{RGB}{0, 127, 0}
\definecolor{hot_desaturated4}{RGB}{255, 255, 0}
\definecolor{hot_desaturated5}{RGB}{255, 96, 0}
\definecolor{hot_desaturated6}{RGB}{107, 0, 0}
\definecolor{hot_desaturated7}{RGB}{224, 76, 76}
\pgfplotsset{
colormap={hotDesat}{
color(0)={hot_desaturated0}
color(0.143)={hot_desaturated1}
color(0.285)={hot_desaturated2}
color(0.429)={hot_desaturated3}
color(0.571)={hot_desaturated4}
color(0.714)={hot_desaturated5}
color(0.857)={hot_desaturated6}
color(1)={hot_desaturated7}
}
}

\definecolor{France0}{RGB}{37, 91, 207}
\definecolor{France1}{RGB}{200, 214, 243}
\definecolor{France2}{RGB}{255,255,255}
\definecolor{France3}{RGB}{243,200,200}
\definecolor{France4}{RGB}{207,37,37}
\pgfplotsset{
colormap={France}{
color(0)={France0}
color(0.25)={France1}
color(0.5)={France2}
color(0.75)={France3}
color(1)={France4}
}
}

\definecolor{Mexico0}{RGB}{28, 155, 68}
\definecolor{Mexico1}{RGB}{198, 230 ,208}
\definecolor{Mexico2}{RGB}{255,255,255}
\definecolor{Mexico3}{RGB}{230, 198, 198}
\definecolor{Mexico4}{RGB}{155, 28, 28}
\pgfplotsset{
colormap={Mexico}{
color(0)={Mexico0}
color(0.25)={Mexico1}
color(0.5)={Mexico2}
color(0.75)={Mexico3}
color(1)={Mexico4}
}
}

\definecolor{MyBuRd0}{RGB}{37, 91, 207}
\definecolor{MyBuRd1}{RGB}{200, 214, 243}
\definecolor{MyBuRd2}{RGB}{243,200,200}
\definecolor{MyBuRd3}{RGB}{207,37,37}
\pgfplotsset{
colormap={MyBuRd}{
color(0)={MyBuRd0}
color(0.33)={MyBuRd1}
color(0.66)={MyBuRd2}
color(1)={MyBuRd3}
}
}

\definecolor{BkWtRd0}{RGB}{0, 0, 0}
\definecolor{BkWtRd1}{RGB}{191, 191, 191}
\definecolor{BkWtRd2}{RGB}{255, 255, 255}
\definecolor{BkWtRd3}{RGB}{243, 200 ,200}
\definecolor{BkWtRd4}{RGB}{207,37,37}
\pgfplotsset{
colormap={BkWtRd}{
color(0)={BkWtRd0}
color(0.25)={BkWtRd1}
color(0.50)={BkWtRd2}
color(0.75)={BkWtRd3},
color(1)={BkWtRd4}
}
}

\pgfplotsset{
colormap={BuWt}{
color(0)={RYB2}
color(1)={BkWtRd2}
}
}

\definecolor{NewBuOr0}{RGB}{37, 91, 207}
\definecolor{NewBuOr1}{RGB}{200, 214, 243}
\definecolor{NewBuOr2}{RGB}{249, 210, 208}
\definecolor{NewBuOr3}{RGB}{232, 74, 69}
\pgfplotsset{
colormap={NewBuOr}{
color(0)={NewBuOr0}
color(0.33)={NewBuOr1}
color(0.66)={NewBuOr2}
color(1)={NewBuOr3}
}
}

\definecolor{NewUIUC0}{RGB}{19, 41, 75}
\definecolor{NewUIUC1}{RGB}{72.25, 49.25, 73.5}
\definecolor{NewUIUC2}{RGB}{125.5, 57.5, 72.}
\definecolor{NewUIUC3}{RGB}{178.75, 65.75, 70.5}
\definecolor{NewUIUC4}{RGB}{232, 74, 69}
\definecolor{NewUIUC5}{RGB}{237.75, 119.25, 115.5}
\definecolor{NewUIUC6}{RGB}{243.5, 164.5, 162.}
\definecolor{NewUIUC7}{RGB}{249.25, 209.75, 208.5}
\definecolor{NewUIUC8}{RGB}{255, 255, 255}

\pgfplotsset{
colormap={NewUIUC}{
color(0)={NewUIUC0}
color(0.125)={NewUIUC1}
color(0.25)={NewUIUC2}
color(0.375)={NewUIUC3}
color(0.5)={NewUIUC4}
color(0.625)={NewUIUC5}
color(0.75)={NewUIUC6}
color(0.875)={NewUIUC7}
color(1)={NewUIUC8}
}
}

\definecolor{BkRdWt0}{RGB}{0, 0, 0}
\definecolor{BkRdWt1}{RGB}{219, 91, 91}
\definecolor{BkRdWt2}{RGB}{255, 255, 255}
\pgfplotsset{
colormap={BkRdWt}{
color(0)={BkRdWt0}
color(0.5)={BkRdWt1}
color(1)={BkRdWt2}
}
}


==> old/garbage.tex <==
\section{Software Description}

\subsection{Goal}

For combustion simulations, we seek source code to evaluate $\{ S_{i} \}_{i = 1}^{N}$ through $\{ \dot{\omega}_{i} \}_{i = 1}^{N}$ per the equations in Section~\ref{sec:chemistry_equations}. In state-of-the-art reacting flow simulations, source terms need to be evaluated at over $100\times10^{6}$ points per time step, so their efficient evaluation is critical to reduce time to solution. Cantera provides $\{ \dot{\omega}_{i} \}_{i = 1}^{N}$ in~\eqref{production_rates}, through simple code such as the Python example of Figure~\ref{fig:ct_source_terms}, where \texttt{mech\_file} is a Cantera input file for the combustion mechanism, and the variables $e$--\texttt{int\_energy}, $\rho$--\texttt{density}, $\{ Y_{i} \}_{i = 1}^{N}$--\texttt{mass\_fractions} are available in the simulation. The simplicity of this code obviously makes it attractive. However, Cantera's goal is to provide a broad range of capabilities to model reacting flows, not fast evaluation in a large-scale simulations. This introduces drawbacks and challenges for high-performance reacting-flow simulations that will be discussed next.

%% \begin{itemize}
%% \item Cantera imposes strong assumptions on inputs
%%   \begin{itemize}
%%   \item \texttt{int\_energy}, \texttt{density}, \texttt{mass\_fractions}
%%     \begin{itemize}
%%     \item Pointwise quantities, stored as 64-point floating point numbers in memory
%%     \item No operation in Section~\ref{sec:chemistry_equations} prevents from inputs from being multi-dim arrays, or even more elaborate objects (as will be discussed in the context of computational graphs)
%%     \end{itemize}
%%   \item Conditions subsequent calculations
%%     \begin{itemize}
%%     \item Implemented as deeply nest loops and conditions
%%     \item Inefficient when executed on GPUs
%%     \end{itemize}
%%   \item Limits analysis and added capabilities
%%     \begin{itemize}
%%     \item Specifically, constructing and analyzing computational graphs
%%       \begin{itemize}
%%       \item At the heart of automatic differentiation, code transformations
%%       \end{itemize}
%%     \end{itemize}
%%   \end{itemize}
%% \end{itemize}

%% \begin{itemize}
%% \item Code generation
%%   \begin{itemize}
%%   \item Relax constraints on inpus:
%%     \begin{itemize}
%%     \item Expressions of~\ref{sec:chemistry_equations} do not involve specific operations that prevent inputs from being multi-dimensional arrays---or even array abstractions
%%     \end{itemize}
%%   \item Generated code can be designed to be \textit{traceable}
%%   \item Retain Cantera's comprehenssiveness, without enhancing speed, and enhancing portability (to e.g., heterogeneous machines)
%%   \end{itemize}
%% \end{itemize}

%% We can avoid this by implementing only what is needed in a simulation based on input provided by Cantera or similar comprehensive thermochemistry engine. (\textit{Prometheus}, from which the package name derives, was a mythical figure who stole fire from the gods.) Resulting source code is, of course, utterly dependent upon Cantera \textit{in its current incarnation}, but it is lightweight and faster than full-library calls, as will be quantified in Section~\ref{subsec:performance}. Pyrometheus automates this approach as a preprocessing step, making it straightforward to switch mechanisms while retaining Cantera's powerful comprehensiveness and without sacrificing speed or portability. As we shall show, the chemical source term routine is expressed in a handful of expressions that are evaluated in a straighforward sequence, which facilitates automation. We exploit this in a template-based strategy to generate lightweight code.

As mentioned in Section~\ref{sec:intro}, one principal drawback of Cantera (and related libraries) is that it imposes strong assumptions on inputs \texttt{int\_energy}, \texttt{density}, and \texttt{mass\_fractions} (Figure~\ref{fig:ct_source_terms}). These inputs are assumed to be pointwise quantities, stored in memory as 64-point floating-point numbers. These assumptions further condition subsequent thermochemistry calculations (implemented as classes, deeply-nested loops, and conditionals), performance, and capabilities, as will be discussed next. For example, given~\ref{fig:ct_source_terms}, it is attractive to use directive-based approaches (e.g., OpenACC or OpenMP) for computing on GPUs. However, compilers cannot vectorize and optimize the deeply nested loops that compute species net production rates~\cite{ref:BarweyPC}. Furthermore, computational graphs cannot be traced across libraries due to the imposed data types. Such graphs form the basis for automatic differentiation and useful optimization methods for both CPU and GPU computing, such as just-in-time compilation and code re-expressions that will be illustrated in Section~\ref{sec:illustrative_examples}.

Constraints on inputs are relaxed through code generation, while retaining the joint goals of differentiable and performant code. The expressions of Section~\ref{sec:chemistry_equations} do not involve any specific operation that would prevent \texttt{int\_energy}, \texttt{density}, and \texttt{mass\_fractions} from being, for example, multi-dimensional arrays of arbitrary types---or even array abstractions. This can easily be infused into the code, so long as a \textit{context} for arithmetic, broadcasting, and nonlinear functions can be provided to the generated code.  Furthermore, source-term evaluation (summarized in steps in Figure~\ref{fig:pyro_source_term_eval_sequence}) does not require storing and updating an internal state. Thus, only the operations that express the chemistry need to be coded. The advantage of this approach is twofold: (i) the generated code is independent on input types, and (ii) it is \textit{traceable}. This means that external tracing packages, with their specific data structures, can be applied to the generated code to construct computational graphs. These properties are to be imbued into the code generation approach, as shown next.

\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.9,page=1]{Figures/pdf/fig_ct_source_terms.pdf}
    \caption{Evaluation of net production rates with Cantera in Python.}
    \label{fig:ct_source_terms}
  \end{center}
\end{figure}

\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.9,page=1]{Figures/pdf/fig_pyro_source_term_procedure.pdf}
    \caption{High-level representation of source-term evaluation. The symbols are: $\rho$ the density, $T$ the temperature, $\bvec{y}$ the mass fractions, $\bvec{C}$ the concentrations, $\bvec{K}$ the equilibrium constants, $\bvec{k}$ the rate coefficients, $\bvec{R}$ the reaction rates, and $\bvec{\omega}$ the species net production rates.}
    \label{fig:pyro_source_term_eval_sequence}
  \end{center}
\end{figure}

\subsection{Code Template}\label{subsec:code_template}

It is useful to break down the source-term computation into: (i) a sequence of evaluation; and (ii) the evaluated expressions themselves. The sequence of evaluation, illustrated in Figure~\ref{fig:pyro_source_term_eval_sequence}, is mechanism independent. Expressions are independent of the number of species and reactions, and they are typically small in number (for hydrocarbon combustion, rarely more than 10). As a consequence, the resulting code varies little in structure across mechanisms. Even within it, many lines will be similar, with small differences in, for example, $A_{j}$, $b_{j}$, and $\theta_{a,j}$ coefficients in~\eqref{rate_coeff} or array indices. This motivates a code template.

An example Python template is provided in Figure~\ref{fig:pyro_template}. Separate templates (\texttt{path/to/pyrometheus/src/codegen/}), with consistent naming and ordering of functions, are provided for Python and \Cpp{}, with a Fortran template provided to guide extensions to other languages. In Python, the template is structured as a class (while the \Cpp{} and Fortran templates represent a structure and a module). Member variables that are mechanism parameters (e.g., number of species $N$) and physical constants (e.g., universal gas constant $\mathscr{R}$). Member functions provide capability to execute the sequence of steps in Figure~\ref{fig:pyro_source_term_eval_sequence}, as will be shown in Section~\ref{sec:illustrative_examples}, but also general mixture thermodynamics (e.g., compute the pressure per~\eqref{eos}). Design choices that make the generated code traceable are discussed next, followed by the template's elements.

As stated, a goal is to infuse the generated code with traceability, which in turn enables automatic differentiation, and code optimization (these capabilities will be showcased through example in Section~\ref{sec:illustrative_examples}). For this, the templated \texttt{Thermochemistry} class of Figure~\ref{fig:pyro_template} abstracts the operations for source-term computation, and does not store nor modify internal states during source-term computation. Further, note that the \texttt{Thermochemistry} class takes an \textit{array context} \texttt{usr\_np} upon construction (line 3 of Figure~\ref{fig:pyro_template}) by design. This array context is an abstraction that allows to operate on NumPy-like arrays. It must provide the broadcasting rules, high-level mathematical functions (specifically \texttt{exp} and \texttt{log}), and a function for conditional evaluation (\texttt{where}). So long as these requirements are met, the generated code can operate on inputs \texttt{density}, \texttt{temperature}, and \texttt{mass\_fractions} independent on their type. These could be pointwise quantities, multi-dimensional arrays, or array-like objects from array-libraries with tracing capabilities to compute and exploit the computational graph of the generated code. This design choice at the template level guarantees the sought-after capabilities. 

The Mako library renders the template into useful code by replacing templated lines, wrapped in $\texttt{\$\{\}}$, with mechanism-specific values and expressions. For this, it takes as input a Cantera solution object $\texttt{sol}$ (Figure~\ref{fig:ct_source_terms}). This object contains the mechanism-specific parameterization that includes the number of species $N$, molecular weights $\{ W_{i} \}_{i = 1}^{N}$, rate-coefficient pre-exponentials $\{ A_{j} \}_{j = 1}^{M}$, and related parameters. In Figure~\ref{fig:pyro_template}, orange text indicates parameter substitution from Cantera. When the template is rendered, template elements $\texttt{\$\{sol.*\}}$ take on specific values from Cantera. For example, in line 3, for a mechanism with, say, the $N = 9$ species of hydrogen combustion, $\texttt{\$\{sol.n\_species\}}$ simply becomes $\texttt{9}$. 
  
%% \todo{I don't know what this means.  What comes from Cantera?  How?  How is that done? You need a bit more here.  Fill out the paragraph.}\

Lines in red represent \textit{expression-generating functions}. These create code for the symbolic expressions of Section~\ref{sec:chemistry_equations}, such as~\eqref{production_rates},~\eqref{reaction_rates}, and~\eqref{rate_coeff}. The necessary expression-generating functions to implement standard combustion thermochemistry are provided in \texttt{path/to/pyrometheus/src/chem\_expr.py}; these have been used to generate code for the comprehensive (containing $C0--C4$ species) USC-II mechanism, with $N = 111$ species and $M = 784$ reactions~\cite{ref:Wang2007}. The expression-generating function for the Arrhenius rate coefficient~\eqref{rate_coeff} is shown in Figure~\ref{fig:pyro_expressions}~(a) (\texttt{path/to/pyrometheus/pyrometheus/chem\_expr.py}). Users seeking to implement less conventional expressions (as for ionization or electronic-excitation reactions) can use these as a guide. As will be discuss, these are independent of template language, so such extensions are straightforward. Note that each expression-generating function creates code for particular species or reactions, typically producing a single line of code. They are called for all species and reactions in a mechanism via template loops, colored brown in Figure~\ref{fig:pyro_template}.

Expression-generating functions, illustrated in Figure~\ref{fig:pyro_expressions} for $k_{j}$~\eqref{rate_coeff} and $\dot{\omega}_{i}$~\eqref{production_rates}, leverage Pymbolic for the symbolic return field~\cite{ref:pymbolic}. Pymbolic can natively create expressions for Python and \Cpp{}. Because these can be easily manipulated, conversions are provided to generate Fortran code. For example, in Figure~\ref{fig:pyro_expressions}~(b), the generated expression can be converted to Fortran by simply replacing brackets with parentheses, and increasing indices by one. Thus, Pyrometheus can provide thermochemistry code in multiple languages without having to modify the provided expression-generating functions. Language specificity is thus fully placed on the template. To switch between generated-code languages, we provide language-specific generator modules, as shown in Figure~\ref{fig:pyro_language_modules}. All modules are imported with Pyrometheus with the standard Python \texttt{import} command. Each one contains the corresponding template, and functions to render it, write it to a file, and to instantiate it (for Python). Thus, to select the output language, users simply need to invoke the corresponding module, as will be shown in the code-generation examples provided in Section~\ref{sec:illustrative_examples} (Figures~\ref{fig:pyro_codegen_py} and~\ref{fig:pyro_codegen_cpp}).

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_language_modules.pdf}
    \caption{Pyrometheus code generation in Python.}
    \label{fig:pyro_language_modules}
  \end{center}
\end{figure}

%\todo{I understand this better, but you should still say a bit more about the user needs do, how they figure out what they need to do, etc.  Or are they provided by Pyrometheus?}

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=0.9,page=1]{Figures/pdf/fig_pyro_template.pdf}
    \caption{Simplified version of the Pyrometheus Python Thermochemistry template. Text in orange, such as in lines 3 through 5, represents variables that are populated from Cantera.}
    \label{fig:pyro_template}
  \end{center}
\end{figure}

%% Expression-generating functions link the equations of Section~\ref{sec:chemistry_equations} with code. Figure~\ref{fig:pyro_rate_coeff_expr} shows an example for the Arrhenius rate coefficient~\eqref{rate_coeff}, as provided in the \texttt{chem\_expr.py} file. Expression-generating functions are contained in \texttt{path/to/pyrometheus/src/chem\_expr.py} and leverage Pymbolic for the symbolic return field~\cite{ref:pymbolic}. Pymbolic can create expressions for Python and \Cpp\,, and can be easily\todo{This isn't clear to me.  Would this be a significant additional Pymbolic?  A small one?}\ extended to convert output to Fortran. Thus, Pyrometheus can provide thermochemistry code in multiple languages without having to modify the provided expression-generating functions.\todo{I don't see where you switch between C++ and Python.}\

\begin{figure}
     \begin{center}
     \subfloat[][Arrhenius rate coefficient~\eqref{rate_coeff}.]{\includegraphics[scale=0.8, page=2]{Figures/pdf/fig_pyro_expressions.pdf}}\\
     \subfloat[][Species net production rate~\eqref{production_rates}.]{\includegraphics[scale=0.8, page=1]{Figures/pdf/fig_pyro_expressions.pdf}}
     \caption{Expression-generating functions, with examples corresponding to the San Diego mechanism.}
     \label{fig:pyro_expressions}
     \end{center}
\end{figure}

\subsection{Chemical Jacobians}\label{subsec:jacobians}

The immediate goal is to provide code to compute chemical Jacobians,
\begin{equation}\label{eq:pyro_jacobian}
  \mathbf{J}_{ij} = \pop{\dot{\omega}_{i}}{Y_{j}},\qquad i = 1,\,\dots\,,N,\qquad j = 1,\,\dots,\, N,
\end{equation}
from Pyrometheus implementations for $\{ \dot{\omega}_{i} \}_{i = 1}^{N}$. There are multiple routes to achieve this. At first, it may seem natural to generate code for each entry of~\eqref{pyro_jacobian}, just as for for the source terms. However, this would involve many more expressions, which would have to be hand-coded, either provided in the package or requested of the user. It would also increase the length and complexity of the templates. To be efficient, it would also require consideration of the order in which expressions are evaluated to avoid overhead and unneeded repeated evaluation of some factors~\cite{ref:Niemeyer2017}.

Another approach consists of finite-difference approximations, but these introduce numerical error, which can be difficult to control in a way that satisfies accuracy goals. In contrast, AD provides exact Jacobians~\cite{ref:Verma2000}. Established AD libraries (e.g., Jax for Python) are effective for traceable routines, such as those coded by Pyrometheus. As extensively discussed, AD compatibility is infused into the code-generation procedure. In Python, AD enabled through the array context, which is an input to the generated class, as discussed. In the example provided in Section~\ref{subsec:compute_jacobians}, the Jax NumPy array context is used. Operations on Jax NumPy arrays are traced and derivatives assembled; the Jacobians~\eqref{pyro_jacobian} is then provided through Jax driver routines. Jax is by no means the only option for AD for Python (one alternative being Functorch). It is adopted here for its dual AD and just-in-time (JI) compilation capabilities, which will be jointly demonstrated on Pyrometheus-generated code in Section~\ref{subsec:autoignition_cpu}.

\textcolor{red}{To allow for AD in \Cpp{}, the generated code is expressed in terms of \textit{generic types}, as shown in Figure~\ref{fig:pyro_cpp_ad}. These are place-ins that are replaced during execution by: (i) conventional types (e.g., \texttt{double}) to interface with a flow solver; or (ii) AD-specific types to compute derivatives. AD considerations are not infused into Fortran-generated code, as the authors are unaware of AD packages for Fortran code.}

\todoECG{The previous paragraph needs work, and the corresponding code does too.}

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=0.9,page=1]{Figures/pdf/fig_pyro_cpp_template.pdf}
    \caption{Simplified version of the Pyrometheus \Cpp{} thermochemistry template, illustrating generic types for AD.}
    \label{fig:pyro_cpp_ad}
  \end{center}
\end{figure}

%% AD is based on the recognition that code is simply a long list of elementary operations with known derivatives on independent variables~\cite{ref:Verma2000}. Broadly, AD tracks these operations, computes their derivatives, and assembles them into desired derivatives (e.g.,~\eqref{pyro_jacobian}) via the chain rule. For AD packages to track and record elementary operations, they implement their own data types and algebraic functions (e.g., $\texttt{exp}$). For our generated code to be compatible with AD, it must be able to handle multiple data types and their corresponding arithmetic. In Python, the generated thermochemistry class takes as input an arithmetic library, which by default is set to NumPy. To enable AD, the user must pass Jax NumPy instead, so as to use Jax AD capabilities, as will be illustrated in Section~\ref{sec:illustrative_examples}

\subsection{Installation}\label{subsec:installation}

Pyrometheus can be downloaded through git:
\begin{equation*}
  \texttt{git clone https://github.com/pyrometheus/pyrometheus.git},
\end{equation*}
which will create a directory called \texttt{pyrometheus} containing the code. To install the code, the user should move into this directory and, from command line, run
\begin{equation*}
  \texttt{python setup.py install}.
\end{equation*}
The \texttt{setup.py} script checks for multiple dependencies, the key ones being: Cantera, Pymbolic, Mako, and pytest. If the user is missing any of these, the script will download and install these.

\subsection{Testing and Verification Suite}\label{subsec:testing_suite}

The testing suite compares Pyrometheus with Cantera, to which it should agree within the limits of computational precision. Cantera itself is well-established, and is extensively tested upon installation. The Pyrometheus testing suite is summarized in Table~\ref{tab:pyro_tests}. In the example here, calculations are conducted for an ethylene-combustion mechanism with 32 species and 206 reactions~\cite{ref:Luo2012}. This mechanism contains many thermochemistry expressions needed broadly in reacting flow simulations.

\begin{table}[H]
  \begin{center}
    \begin{tabular}{l l}
      \hline
      Test Name & Description\\
      \hline
      \texttt{test\_get\_temperature}        & Temperature computation via\\
                                             & Newton method~\eqref{newton_temperature} \\
      \texttt{test\_get\_thermo\_properties} & Species thermodynamics~\eqref{gibbs} and~\eqref{nasa_poly} \\
      \texttt{test\_get\_rate\_coefficients} & Rate coefficients~\eqref{rate_coeff} \\
      \texttt{test\_get\_kinetics}           & Net species productions rates~\eqref{production_rates}\\
                                             & and reaction rates of progress~\eqref{reaction_rates}\\
      \texttt{test\_autodiff\_accuracy}      & AD Jacobians~\eqref{pyro_jacobian}\\
                                             & versus finite-difference approximations~\eqref{pyro_j_fd}\\
      \hline
    \end{tabular}
    \caption{Summary of Pyrometheus testing suite, which is part of the distribution.}
    \label{tab:pyro_tests}
  \end{center}
\end{table}

Species specific heats~\eqref{nasa_poly_cp} and Arrhenius rate coefficients~\eqref{rate_coeff} are computed over a combustion-relevant temperature range $T \in \psq{500, 2500}$ $\mathrm{K}$. Major-species thermodynamics, as given by NASA polynomials~\eqref{nasa_poly} and~\eqref{nasa_poly_cp}, are shown in Fig.~\ref{fig:pyro_thermo_poly}, and Arrhenius rate coefficients~\eqref{rate_coeff} are shown in Fig.~\ref{fig:pyro_rate_coeffs}. Both match Cantera to within machine precision, as no approximations are made, and all constants are implemented to the same precision as in Cantera.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_thermo_poly_verif.pdf}
    \caption{Species specific heat, enthalpy, and entropy, as given by NASA polynomials~\eqref{nasa_poly_cp} and~\eqref{nasa_poly}, for selected major species computed with \solidrule\, Pyrometheus, and $\bullet$ Cantera for verification.}
    \label{fig:pyro_thermo_poly}
  \end{center}
\end{figure}

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_rate_coeffs_temp_verif.pdf}
    \caption{Arrhenius forward and reverse rate coefficients for selected reactions computed with \solidrule\, Pyrometheus, and $\bullet$ Cantera for verification.}
    \label{fig:pyro_rate_coeffs}
  \end{center}
\end{figure}

Since Cantera does not provide reference Jacobians, we rely on finite difference for verification:
\begin{equation}\label{eq:pyro_j_fd}
  \mathbf{J}_{ij} \approx \mathbf{J}_{ij}^{\mathrm{FD}} = \frac{1}{\Delta Y}\psq{ \dot{\omega}_{i}(\bvec{Y} + \Delta Y \bvec{e}_{j}) - \dot{\omega}_{i}(\bvec{Y}) },
\end{equation}
where $\Delta Y$ is a mass-fraction perturbation, and $\bvec{e}_{j}$ is the unit vector indicating the $j^{\mathrm{th}}$ species. If $\mathbf{J}^{\mathrm{AD}} = \mathbf{J}$, then~\eqref{pyro_j_fd} should converge to it until the limit of computational precision is reached as
\begin{equation}\label{eq:pyro_j_err}
  \varepsilon = \| \mathbf{J}^{\mathrm{AD}} - \mathbf{J}^{\mathrm{FD}} \|_{F} \sim \Delta Y
\end{equation}
where $\|\cdot\|_{F}$ is the Frobenius norm. Here, we verify $\mathbf{J}^{\mathrm{AD}}$ against $\mathbf{J}^{\mathrm{FD}}$~\eqref{pyro_j_fd} for the 32-species ethylene mechanism. The input composition is chosen from an auto-ignition simulation, for which details are provided elsewhere~\cite{ref:Cisneros2021}. Specifically, we use the mixture composition at the time of maximum $Y_{\ce{CH3}}$. This defined a nominal ignition~\cite{ref:SanchezWilliams2014}, and therefore challenging, state to test Jacobians. Figure~\ref{fig:pyro_jacobian} shows $\| \mathbf{J}^{\mathrm{AD}} - \mathbf{J}^{\mathrm{FD}} \|_{F}$ convergence with $\Delta Y$. For $\Delta Y$ decreasing from $10^{-10}$,~\eqref{pyro_j_err} grows due to round-off error in the difference in the numerator. For $\Delta Y > 10^{-10}$,~\eqref{pyro_j_err} $\varepsilon \sim \Delta Y$, asserting that $\mathbf{J}^{\mathrm{AD}} = \mathbf{J}$.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_jacobian.pdf}
    \caption{Finite-difference error in the Jacobian with respect to automatically-differentiated Pyrometheus code. The error decreases as $\Delta Y^{-1}$, as expected, supporting the correctness of $\mathbf{J}_{\mathrm{AD}}$.\todo[inline]{I think you should run it to large $\Delta Y$, until that fails to be linear.  More decades the better!}}
    \label{fig:pyro_jacobian}
  \end{center}
\end{figure}

\section{Illustrative Examples}\label{sec:illustrative_examples}

This section shows how to use Pyrometheus to compute chemical source terms in~\eqref{massfrac_ode} and Jacobians~\eqref{pyro_jacobian} via generation and execution. We provide example code for each. These examples are also provided with the distribution in \texttt{path/to/pyrometheus/examples}; this section serves as a corresponding guide. The first example shows how to generate code for the chemical source terms in Python and \Cpp{}. With generated code, examples on how to compute chemical source terms is provided. These are then put together to conduct autoignition simulations that integrate~\eqref{massfrac_ode}. Performance is quantified and compared with Cantera. The section ends with an example on how to compute chemical source terms on GPUs through generated-code re-expressions.

\subsection{Generating Code for Chemical Source Terms}

For Python, the generation procedure is shown in Figure~\ref{fig:pyro_codegen_py}; comments therein provide a brief explanation for corresponding lines. The key dependency in this example is the Cantera solution object~\texttt{sol}, which the user must instantiate as per Figure~\ref{fig:ct_source_terms}, though once Pyrometheus code is generated, it is no longer needed. Line 3 generates the thermochemistry class; the template is populated with mechanism parameterization in \texttt{sol}, as described in Section~\ref{subsec:code_template}. Line 4 instantiates a thermochemistry object \texttt{pyro\_gas} with NumPy as the array context. This choice is enough to simply compute net production rates, either from pointwise quantities or arrays that represent grids, as will be shown in Section~\ref{subsec:compute_source_terms}.

Multi-language generation is demonstrated for \Cpp{} in Figure~\ref{fig:pyro_codegen_cpp}. Per Section~\ref{subsec:code_template}, the generation modules of Figure~\ref{fig:pyro_language_modules} are the mechanism by which users select language, and in Figure~\ref{fig:pyro_codegen_cpp}, the \texttt{codegen.cpp} module creates the thermochemistry code as a string (line 2), which is then written to a file (line 3). Users can follow this same procedure, with \texttt{codegen.fortran} to generate Fortran code.

%% In line 5, source-term computation is encapsulated in a function that will serve for Jacobian computation. In lines 6 \& 7 show evaluate thermodynamic state relations to obtain the temperature (through the Newton method) and the density. With these, the net production rates~\eqref{production_rates} are computed in line 8.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_py_codegen.pdf}
    \caption{Pyrometheus code generation in Python.}
    \label{fig:pyro_codegen_py}
  \end{center}
\end{figure}

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_cpp_codegen.pdf}
    \caption{Pyrometheus code generation in \Cpp. The corresponding language swap (with respect to Figure~\ref{fig:pyro_codegen_py}) is highlighted in red in line 2.}
    \label{fig:pyro_codegen_cpp}
  \end{center}
\end{figure}

%\todo[inline]{What is Jax?}
%\todo[inline]{Same comments as above:  what exactly are we doing here?  Why does the use need to do?  How would the output be used?  Should have an example calling code?}

\subsection{Computing Chemical Source Terms}\label{subsec:compute_source_terms}

The goal is to evaluate chemical source terms~\eqref{production_rates} using the Pyrometheus thermochemistry object of the preceding example. To compute species net production rates, the temperature must be computed from the mixture internal energy and mass fractions using the Newton method~\eqref{int_energy}--\eqref{newton_iteration}, so this is illustrated first.

The example code is shown in Figure~\ref{fig:pyro_source_terms}. It uses the 32-species ethylene mechanism of the verification cases in Section~\ref{subsec:testing_suite}, but the procedure is mechanism-independent. Lines 1 through 5 set the necessary variables to compute the source terms: density, internal energy, and species mass fractions. These correspond to equivalence ratio
\begin{equation}\label{eq:equiv_ratio}
  \phi = \frac{\nu\,Y_{\ce{C2H4}}}{Y_{\ce{O2}}} = 1,
\end{equation}
where $\nu = 3\,W_{\ce{O2}}/W_{\ce{C2H4}}$ and temperature $T = 1500\,\mathrm{K}$. Though here hardcoded (for illustration), in practice their values would typically come from the flow solver, corresponding to the mixture state at a grid point. 

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_source_terms.pdf}
    \caption{Pyrometheus code generation in Python.}
    \label{fig:pyro_source_terms}
  \end{center}
\end{figure}

An initial temperature guess is provided in line 6 to initialize the Newton method~\eqref{int_energy}--\eqref{newton_iteration} (line 7). This returns the temperature corresponding to the given internal energy and mass fractions. It is then used to compute (temperature-dependent) species production rates~\eqref{production_rates} line 8, the key step to meet the goal of computing net production rates for a flow simulation. These values can then returned to the flow solver to advance the simulation state. This procedure translates straightforwardly to other languages.

\textcolor{red}{To demonstrate independence on input types, net production rates are evaluated on simulation grids. For this, a freely-propagating premixed flame simulation (Figure~\textcolor{red}{}~(a)) is conducted with Cantera. Solution fields are represented as NumPy arrays. Pyrometheus-generated code can operate on these, without the need to loop over points in the grid.}

\subsection{Computing Jacobians}\label{subsec:compute_jacobians}

Recall that the generated code is designed to be compatible with established AD libraries. This is achieved through the generated code's traceability. Here, AD compatibility is illustrated using Jax and its Jax NumPy array context. However, while examples are crafted around Jax, Pyrometheus is not overly constrained by this choice, and integrating other AD packages should not require extensive modification so long as a corresponding array context is provided.

Figure~\ref{fig:pyro_jax} illustrates Jacobian computation using Jax. The Jax array context, and the AD Jacobian-computation driver \texttt{jacfwd} (the use of which is described in what follows), are imported in lines 1 and 2. The thermochemistry class is generated in line 3 through standard procedure, and the AD compatible object is instantiated in line 4 by setting the Pyrometheus array context to be Jax Numpy (\texttt{jnp}). The argument to the \texttt{jacfwd} driver is function it will differentiate---the \texttt{chemical\_source\_term} function of line~5. This function is identical in body to that of Figure~\ref{fig:pyro_source_terms}, line~8, though uses the \texttt{pyro\_gas} with \texttt{jnp} array context. Per line~10, mass fractions used for computation are now \texttt{jnp} arrays; these are initialized with the NumPy array of Figure~\ref{fig:pyro_source_terms}, lines~3--6. The corresponding Jacobian is then computed in line 9.

%% This is shown in line 6, a Jax array is populated using the NumPy array for the mass fractions, and the Jacobian is then computed in line 7 using the Jax function \texttt{jacfwd} on \texttt{chemical\_source\_term} of line 5 in Figure~\ref{fig:pyro_codegen}. 

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_jax.pdf}
    \caption{Instantiation of a AD-enabled Pyrometheus thermochemistry class in Python using Jax NumPy. Key instantiation using Jax Numpy is highlighed in red in line 4. The \texttt{density} comes from the flow solver, and \texttt{temperature} from e.g., Figure~\ref{fig:pyro_source_terms}.}
    \label{fig:pyro_jax}
  \end{center}
\end{figure}

\subsection{Zero-dimensional Auto-ignition Simulations on CPUs}\label{subsec:autoignition_cpu}

This example illustrates how to use Pyrometheus-generated code to predict homogeneous auto-ignition of a combustible mixture. It targets CPU execution of Python-generated code, and showcases the properties that enable corresponding simulations. In particular, the example demonstrates that the generated code can be automatically differentiated for implicit time marching, and compiled for performance. Here, we predict ignition time of a homogeneous ethylene--air reactor by integrating the system of Equations~\eqref{massfrac_ode}. Reactions are modeled with a $32$-species, $206$-reactions skeletal mechanism~\cite{ref:Luo2012}. The initial condition $\{Y_{k}^{0}\}_{k = 1}^{N}$ has an equivalence ratio $\phi = 1$ (Equation~\eqref{equiv_ratio}). This stiff system is marched implicitly via standard Crank-Nicolson with a Newton method.

The stiff system~\eqref{massfrac_ode} is discretized via standard Crank-Nicolson, so
\begin{equation}\label{eq:crank_nicol_rhs}
  \underbrace{ Y_{k}^{m+ 1} - Y_{k}^{m} + \frac{1}{2\Delta t}\pp{ S_{k}^{m + 1} + S_{k}^{m} } }_{\equiv \mathscr{N}_{k}} = 0, 
\end{equation}
where the superscript indicates the time step, and $S_{k} \equiv W_{k}\dot{\omega}_{k} / \rho$. Equation~\eqref{crank_nicol_rhs} is nonlinear through $S_{k}^{m + 1}$, so $Y_{k}^{m + 1}$ is obtained via a standard Newton method
\begin{align}\label{eq:crank_nicol_newton}
  &\psq{Y_{k}^{m + 1}}^{n + 1} = \psq{Y_{k}^{m + 1}}^{n} + \psq{\Delta Y_{k}^{m + 1}}^{n} \\
  &\mathscr{J}_{jk}\pp{\psq{Y_{k}^{m + 1}}^{n}; Y_{k}^{m}, \Delta t}\psq{\Delta{Y}_{k}^{m + 1}}^{n} = -\mathscr{N}_{k}\pp{\psq{Y_{k}^{m + 1}}^{n}; Y_{k}^{m}, \Delta t},
\end{align}
where the superscripted bracket indicates the $n^{\mathrm{th}}$ Newton iteration,
\begin{equation}\label{eq:crank_nicol_jac}
  \mathscr{J}_{jk} \equiv \frac{\partial \mathscr{N}_{j}}{\partial Y_{k}} = \delta_{jk} + \frac{1}{2\Delta t}\mathbf{J}_{jk},
\end{equation}
with $\mathbf{J}$ the chemical Jacobian~\eqref{pyro_jacobian}, and $\delta_{jk}$ the Kronecker delta. The Newton method for each time step is initialized with $\psq{ Y_{k}^{m + 1} }^{0} = Y_{k}^{m}$. 

Figure~\ref{fig:pyro_autoign_sim} shows the Pyrometheus-based implementation of the time integrator~\eqref{crank_nicol_rhs}--\eqref{crank_nicol_jac}. It is based on the Jax NumPy array context, as seen in line \textcolor{red}{2}. As discussed in Section~\ref{subsec:jacobians}, this array context provides automatic differentation capabilities. It also allows for just-in-time (JIT) compilation, as seen in line~\textcolor{red}{3}, a capability that again follows from the generated code's traceability, and which will be explained next. When enabling JIT compilation of a function (e.g., through the \texttt{@jit} decorator per line~\textcolor{red}{3}), Jax transforms the code that operates on Jax arrays into compilable code. In practice, JIT runs the Python code for one time step to trace and transform it into compilable code, and then executes the compiled code. The JIT-compiled Pyrometheus-based code is $16\%$ faster than a Cantera-based implementation of the time integrator.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_autoign.pdf}
    \caption{Pyrometheus-based implementation of the Crank--Nicolson time integrator~\eqref{crank_nicol_rhs}--\eqref{crank_nicol_jac}.}
    \label{fig:pryo_autoign}
  \end{center}
\end{figure}

Figure~\ref{fig:pyro_autoign_sim} shows the time evolution of temperature and  mass fraction of key species. The horizontal dashed line in Figure~\ref{fig:pyro_autoign_sim}~(a) indicates the equilibrium temperature computed with Cantera; by $t = 1,\mathrm{ms}$, the simulation temperature is within $10^{-6}\,\mathrm{K}$ of this equilibrium value. The vertical dashed line in Figure~\ref{fig:pyro_autoign_sim}~(a) indicates the ignition time reported by Luo et al.~\cite{ref:Luo2012} for the full mechanism from which the skeletal is derived, which coincides to within $4\%$ with the time of maximum $Y_{\ce{CH3}}$ from the simulation. These close comparisons validate our calculation.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=1,page=1]{Figures/pdf/fig_autoign_data.pdf}
    \caption{Time evolution of homogeneous reactor state during autoignition: (a) temperature; and (b) mass fractions of key species.}
    \label{fig:pyro_autoign_sim}
  \end{center}
\end{figure}

Simulation data can be further analyzed with Pyrometheus in post-processing. One such example is mechanism reduction through time-scale analysis, with the particular methodology here adopted requiring Jacobian evaluations (as will be explained). \textcolor{red}{Will flesh out more in the next few days.}

\subsection{One-dimensional Flamelet Simulations on CPUs}\label{subsec:flamelet_cpu}

The immediate goal is to demonstrate that Pyrometheus can seamlessly operate on arrays that represent discretization over grids (as in flow simulations), as opposed to pointwise quantities of the previous example. For this, the \textit{flamelet} equations~\textcolor{red}{someref} 
\begin{align}
  &\frac{\chi\rho}{2}\frac{d^{2}\mathbf{q}}{dZ^{2}} + \dot{\mathbf{m}} + \mathbf{f} = \mathbf{0},\label{eq:flamelet_eqns} \\
  &\mathbf{q}(0) = \mathbf{q}_{\mathrm{ox}},\, \mathbf{q}(1) = \mathbf{q}_{\mathrm{fu}}\label{eq:flamelet_bcs}
\end{align}
are solved, with $\mathbf{q} = \{ T,\, Y_{1},\, \dots,\, Y_{N} \}$ the thermochemical state, and $0 \leq Z \leq 1$ the mixture fraction, and $\chi$ its dissipation rate, with $\rho$ evaluated using the equation of state~\eqref{eos} with a prescribed constant pressure. In Equation~\eqref{flamelet_eqns}
\begin{align}
  \dot{\mathbf{m}} = \begin{bmatrix} -\frac{1}{c_{p}}\sum_{k = 1}^{N}W_{k}\dot{\omega}_{k}h_{k} \\ S_{1} \\ \vdots \\ S_{N} \end{bmatrix},\qquad \mathbf{f} = \begin{bmatrix} \frac{\chi\rho}{2}\frac{1}{c_{p}}\pp{ \frac{dT}{dZ}\frac{dc_{p}}{dZ}  + \frac{dT}{dZ}\sum_{k = 1}^{N}c_{p,k}\frac{dY_{k}}{dZ} } \\ 0 \\ \vdots \\ 0 \end{bmatrix},
\end{align}
and $\mathbf{q}_{\mathrm{ox}}$ and $\mathbf{q}_{\mathrm{fu}}$ the boundary states, representing unmixed oxidizer and fuel streams. Equations~\eqref{flamelet_eqns}--\eqref{flamelet_bcs} model the competing effects of chemical reactions and strain, represented by the dissipation rate $\chi$. These are chosen to fulfill the stated goal as they are simpler to implement than other one-dimensional combustion problems (e.g., freely propagating planar flames). The equations~\eqref{flamelet_eqns}--\eqref{flamelet_bcs} are discretized on a uniform grid $\{ Z_{i} \}_{i = 1}^{N_{Z}}$, so
\begin{equation}\label{eq:discrete_flamelet_eqns}
  \vec{\mathscr{F}} = \begin{bmatrix}
    \mathbf{q}_{1} - \mathbf{q}_{\mathrm{ox}} \\
    \frac{\chi_{i}\rho_{i}}{2}\mathbf{L}_{ij}\mathbf{q}_{i} + \dot{\mathbf{m}}_{i} + \mathbf{f}_{i} \\
    \mathbf{q}_{K} - \mathbf{q}_{\mathrm{fu}}
    \end{bmatrix} = \mathbf{0}.
\end{equation}
To solve this nonlinear set of equations, a Newton method is employed:
\begin{align}
  [\mathbf{q}_{i}]^{n + 1} = [\mathbf{q}_{i}]^{n} + [\Delta\mathbf{q}_{i}]^{n}, \label{eq:newton_iter}\\
  \underline{\mathscr{G}}_{ij}[\Delta\mathbf{q}_{j}]^{n} = - \mathscr{F}_{j}, \label{eq:newton_linsys}
\end{align}
where $[\cdot]^{n}$ represents the $n^{\mathrm{th}}$ iteration, and
\begin{equation}
  \underline{\mathscr{G}}_{ij} \equiv \frac{\partial \mathscr{F}_{i}}{\partial \mathbf{q}_{j}},
\end{equation}
obtained through AD as will be shown. To ensure convergence of the Newton method, an initial guess $\{[\mathbf{q}_{i}]^{0}\}_{i = 1}^{N_{Z}}$ that is sufficiently close to the steady-state solution must be provided. This is rarely the case, so the Newton method is complemented with second-order implicit pseudo-time marching to bridge the state from the initial guess to within the radius of convergence of the solution. Details are provided with the distribution in \texttt{examples/steady\_flamelet.py}. 

Equation~\eqref{discrete_flamelet_eqns} is implemented using a Jax NumPy array context, with $\{\mathbf{q}_{i}\}_{i = 0}^{n}$ a two-dimensional $(N+1) \times N_{Z}$ Jax NumPy (\texttt{jnp}) array. This is shown in lines~$7$--$10$ of Figure~\ref{fig:chirho_code}. Thus, the functions that implement $\vec{\mathscr{F}}$ and $\underline{\mathscr{G}}$ return Jax NumPy arrays, as seen in lines $14$--$19$. Note that $\underline{G}$ is implemented by automatically differentiating the Chirhometheus implementation of Equation~\eqref{discrete_flamelet_eqns} (line $19$). This obviates the need of deriving and implementing complex derivatives of the discrete flamelet equations. The system~\eqref{newton_linsys} is solved using Jax NumPy \texttt{linalg}, as shown in line~\textcolor{red}{someline}.

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=0.8,page=2]{Figures/pdf/fig_chirhometheus.pdf}
    \caption{Stripped-down version of Chirhometheus implementation using Jax NumPy arrays to represent thermochemistry on the $Z$ grid.}
    \label{fig:chirho_code}
  \end{center}
\end{figure}

The solution to Equation~\eqref{flamelet_eqns}, as computed with Chirhometheus, is shown in Figure~\ref{fig:chirho_solutions}. This is verified against the established PDRs solver~\cite{ref:Mueller2020}. Chirhometheus and PDRs profiles match to within $2\%$, and this difference can be ascribed to differences in the mechanism files, and the precision with which each code implements its constants (e.g., $\mathscr{R}$ and $\{ W_{i} \}_{i = 1}^{N}$). 

\begin{figure}[H]
  \begin{center}
    \includegraphics[scale=0.8,page=1]{Figures/pdf/fig_chirhometheus_prediction.pdf}
    \caption{Chirhometheus solution to flamelet equations~\eqref{flamelet_eqns}--\eqref{flamelet_bcs}: (a) temperature; and (b) mass fractions of key radicals.}
    \label{fig:chirho_solutions}
  \end{center}
\end{figure}

\subsection{Autoignition Simulations on GPUs}\label{subsec:autoignition_gpu}

\todoECG{Need to get the GPU example done.}

%% \section{Performance}\label{subsec:performance}

%% \todoECG{Skip! There was a bug in this comparison.}

%% Performance is quantified for \Cpp{} code simply via source-term evaluation CPU time, though it is similar for other languages. Pyrometheus-generated code is benchmarked against Cantera. Three representative mechanisms are used: the San Diego mechanism for hydrogen combustion~\textcolor{red}{someref}, with $9$ species and $24$ reactions; (ii) the UConn mechanism for ethylene combustion, with $32$ species and $206$ reactions~\cite{ref:Luo2012}; and (ii) the GRI-3.0 mechanism for methane combustion, with $53$ species and $325$ reactions~\textcolor{red}{someref}. To avoid including initialization costs, $10^{7}$ source-term computations are conducted, timed, and averaged; results are insensitive to the number of evaluations. Cantera can cache and reuse source terms if temperature and composition do not change, so each of source-term evaluation were taken to have a different $\{ T,\, Y_{1},\, \dots,\, Y_{N} \}$, as would be the case in a reacting flow simulation. For this, we take the states from linear profiles:
%% \begin{align}\label{eq:grid_demons_profiles}
%%   &T(\zeta) = T_{0} + (T_{1} - T_{0})\,\zeta\\
%%   &Y_{i}(\zeta) = Y_{i,0} + (Y_{i,1} - Y_{i,0})\,\zeta,\qquad i = 1,\dots,N,
%% \end{align}
%% where $0 \leq \zeta \leq 1$ is an independent variable, $\{ T_{0},\, T_{1} \}$ and $\{ Y_{i,0}, Y_{i,1} \}_{i = 1}^{N}$ are the temperature and mass fractions at $\zeta = \{0, 1\}$. For this demonstration,
%% \begin{equation}
%%   T_{0} = 1000,\qquad T_{1} = 300\,\mathrm{K},
%% \end{equation}
%% and
%% \begin{equation}
%%   Y_{s, 0} = \begin{cases}
%%     Y_{\mathrm{air},s} & s = \{\ce{O2},\, \ce{N2} \}, \\
%%     0 & \textrm{otherwise}
%%   \end{cases}\,\text{ and } \qquad
%%   Y_{s, 1} = \begin{cases}
%%     1 & s = \textrm{Fuel}, \\
%%     0 & \textrm{otherwise}
%%   \end{cases},
%% \end{equation}
%% where, depending on the mechanism, $\textrm{Fuel} = \ce{H2}$, $\ce{C2H4}$, or $\ce{CH4}$. Results are summarized in Figure~\ref{fig:pyro_cost}. Pyrometheus clearly provides cost savings with respect to Cantera, and these improve with mechanism size: $26\%$ for San Diego, $61\%$ for UConn, and $57\%$ for GRI-3.0.

%% \begin{figure}[H]
%%   \begin{center}
%%     \includegraphics[scale=1,page=1]{Figures/pdf/fig_pyro_cost.pdf}
%%     \caption{Source-term evaluation cost comparison between Pyrometheus-generated code and Cantera. The percentages represent corresponding Pyrometheus speed-up.}
%%     \label{fig:pyro_cost}
%%   \end{center}
%% \end{figure}

%% \subsubsection{GPU Computing of Chemical Source Terms}\label{subsub:offloading}

%% \todoECG{This will need to be reworked to use Pytato.}

%% The previous example is revisited in the context of GPU offloading to demonstrate the usefulness of \textit{Python-generated} Pyrometheus code. Individual-mechanism operations are exposed to code transformation tools that re-generate kernels as OpenCL code, which then runs on GPUs.

%% \todo[inline]{Need to flesh this out, having minor issues with the implementation.}

\section{Impact and Additional Discussion}\label{sec:impact}

%% \textbf{This is the main section of the article and the reviewers weight the description here appropriately}\\
%% %
%% \textit{Indicate in what way new research questions can be pursued as a result of the software (if any).}\\
%% %
%% \textit{Indicate in what way, and to what extent, the pursuit of existing research questions is improved (if so).}\\
%% %
%% \textit{Indicate in what way the software has changed the daily practice of its users (if so).}\\
%% %
%% \textit{Indicate how widespread the use of the software is within and outside the intended user group.}\\
%% %

A code-generation approach to implementing combustion thermochemistry has been presented. It is open source, under the MIT lincense, \url{https://github.com/ecisneros8/pyrometheus}, and the release includes a testing suite for verification against Cantera. Extensive documentation is included in the release.  Because it provides (1) lightweight code, (2) in standard languages, and (3) without dependencies, it has the potential to impact any large-scale combustion simulations. Application areas might include (i) turbulent-combustion simulations~\cite{ref:Cisneros2022}; (ii) dynamic adaptive chemistry~\cite{ref:Sun2015}, where multiple sub-mechanisms need to be evaluated on the fly; or (iii) simultaneous model reduction and uncertainty quantification, for which, in fact, an earlier version of the code has already been utilized~\cite{ref:Cisneros2019}.

Pyrometheus is based on a template that reflects chemical kinetics equations, following the natural order of their formulation. The generated code is designed to be traceable, and the computational graph can be exploited for automatic differentation and code optimization. The code is independent of input type, so long as an array context can be provided. Mechanism-specific expressions are generated using Pymbolic, which provides multi-language capability, which should facilitate use and extension. For example, to extend current functionality to other languages, only a new template is needed; the Pyrometheus expression-generating functions need not be modified. Because the generated code is designed to be compatible with automatic differentiation, only code for chemical source terms is generated; the corresponding Jacobians are provided by AD tools. Our Python demonstrations use the established Jax package for simultaneous AD and JIT compilation for performance. Extensions to different expressions to represent additional chemical kinetics (such as plasma or surface chemistry) do no need to explicitly implement corresponding derivatives.

Currently, Pyrometheus implements thermochemistry in multiple reacting-flow solvers: \textit{MIRGE-Com} and \textit{PyFlowCL} in Python, and \textit{PlasCom2} and \textcolor{red}{\textit{WaveletCode}} in \Cpp{}. Preprocessing with Pyrometheus code generation obviates the need to incorporate Cantera or similar engine into the simulation. In direct implementation on CPUs, the overall simulation was 1.6 times faster, including all compressible flow solver and species transport operations. However, GPU-based simulations are the primary motivation, and indeed running on GPUs was hundreds of times faster since dependencies prohibited efficient GPU computation, at least without a significant overhaul of the full library. In \textit{MIRGE-Com}, it is specifically used for offloading thermochemistry to GPUs, for which its generated Python code is regenerated in openCL. This is not possible with standard Cantera. It has also been implemented as an alternative thermochemistry engine in the laminar-flame library PDRs~\cite{ref:Mueller2020}. It is anticipate that it might see wider use with its full release.

One possible extension will be to generate similar code to for other \textit{domain kinetics} (e.g., thermal-nonequilibrium plasma or nuclear kinetics). Similarly, it should be possible to use other engines to drive Pyrometheus. Any engine (e.g., Mutation++ for ionized-gas thermochemistry~\cite{ref:Scoggins2020}) would need to be able to provide just parameterization for (i) species thermodynamics and (ii) reaction kinetics.


==> old/old_design.tex <==
\section{Software Description}\label{sec:design}

\subsection{Goal \& Approach}

\begin{itemize}
\item Motivation: Compute source terms
\item Challenge: Cantera
  \begin{itemize}
  \item Can compute, but cannot offload
  \item Capabilities---computational and analytical---constrained by inputs
    \begin{itemize}
    \item Thermochemical state
      \begin{itemize}
      \item As stated, assumed to be pointwise quantities
      \item GPUs utilization optimized for array computations
      \item Major overhaul required, likely to sacrifice capabilities
      \end{itemize}
    \item Mechanism parameterization
      \begin{itemize}
      \item What is the challenge with this?
      \end{itemize}
    \end{itemize}
  \end{itemize}
\item Approach
  \begin{itemize}
  \item Separate input details from symbolic representation
    \begin{itemize}
    \item Mechanism data
      \begin{itemize}
      \item Cantera already separates: can swap mech\_file and compute for different fuels and rates
      \item Package vs code generation
      \end{itemize}
    \item Thermochemical state
      \begin{itemize}
      \item Produces symbolic view of the math
      \item Enables code transformations for AD and GPU offloading
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

For combustion simulations, we seek source code to evaluate $\{ S_{i} \}_{i = 1}^{N}$ through $\{\dot{\omega}_{i} \}_{i = 1}^{N}$ per the equations in Section~\ref{sec:formulation}. Recall from Section~\ref{sec:introduction} that this code must simultaneously meet two properties: it must (i) be portable to GPUs, for high-performance computing; and (ii) provide exact derivatives, for sensitivity (though also for implicit time marching and time-scale analysis). In this Section Pyrometheus, a novel computational design that meets these goals, is developed in detail.

We use Cantera as a starting point to introduce key notation and concepts, and provide a concrete example of why such libraries do not to serve our goals. Indeed, Cantera provides $\{ \dot{\omega}_{i} \}_{i = 1}^{N}$ in~\eqref{production_rates}, through simple code such as the Python example of Figure~\ref{fig:ct_source_terms}, where \texttt{mech\_file} is a Cantera input file for the combustion mechanism parameterization, and $e$--\texttt{int\_energy}, $\rho$--\texttt{density}, $\{ Y_{i} \}_{i = 1}^{N}$--\texttt{mass\_fractions} characterize the thermochemical state and are available in the simulation. The simplicity of this code obviously makes it attractive but it is not portable to GPUs, at least not readily or without extensive modifications~\cite{ref:Barwey2022}. As state in Section~\ref{sec:introduction}, Cantera assumes its inputs are pointwise quantities, 

\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.8, page=1]{Figures/pdf/fig_ct_source_terms.pdf}
    \caption{Evaluation of net production rates with Cantera in Python.}
    \label{fig:ct_source_terms}
  \end{center}
\end{figure}

Despite these shortcomings, Cantera populates a data structure---the Solution object \texttt{sol}---with mechanism parameterization, and makes it available through a simple, well-documented Python interface. This will be useful in subsequent development: while no computation will be done through Cantera, it will be leveraged to manage mechanism-specific data. Indeed, the formulation of Section~\ref{sec:formulation} is independent of mechanism-specific values, and we will mirror this property in the proposed computational approach.

To overcome the limitations of Cantera (and related libraries) relative to our goals, we will design Pyrometheus to separate the symbolic representation of the thermochemistry (Section~\ref{sec:formulation}) from: (i) mechanism-specific data; and, more importantly, (ii) any details of the inputs to the thermochemistry calculation. The first property will enable automated code generation, while the second allows the generated code to retain a symbolic representation that can be analyzed without sacrificing direct execution. We first introduce the code-generation procedure, based on an outer shell with the overall structure and a symbolic core that generates specific expressions. Then, we introduce the design choices that 

Broadly, there are two approaches to computational design for combustion thermochemistry: (i) package (e.g., Barwey \& Raman~\cite{ref:Barwey2022}); and (ii) mechanism-specific code generation (e.g., Niemeyer et al.~\cite{ref:Niemeyer2017}). Here, we rely on automated code generation to obtain combustion thermochemistry implementations that meet our goals. This approach produces lightweight code only for what is needed in large-scale combustion simulations, though it can be easily extended and generalized.  

%% The Pyrometheus computational design is developed as follows: first, the \textit{symbolic core} that separates the symbolic representation from mechanism data is presented. This is followed by the design choices that enable separating the same symbolic representation from input details. It is explained how this feature in turn enables automatic differentiation and

%% Pyrometheus is written in Python. Its scripting nature allows for a simple  During the code-generation procedure, more complex tasks, such as data management and symbolic manipulation, are offloaded to dedicated packages.  

\subsection{Code Design}

\subsubsection{Code Generation: Code Template \& Symbolic Core}

%% To ensure our combustion thermochemistry implementation meets our goals, we rely on automated code generation. In this way, we can tailor the implementations to have properties that meet our goals---simultanteous computation and symbolic analysis. 

To guide development, we will use a subset of the hydrogen-combustion San Diego mechanism~\cite{ref:Williams2018}, summarized in Table~\textcolor{red}{sometab}. This subset is chosen for its simplicity and importance to combustion: it models the exponential growth of the concentration of radicals \ce{H}, \ce{O} and \ce{OH}~\cite{ref:Sanchez2018,ref:Westbrook1984}. Figure~\textcolor{red}{somefig} shows the corresponding code expressions for equations~\eqref{reaction_rates} (net reaction rates) and~\eqref{rate_coeff} (Arrhenius rate coefficients). It is clear that expressions are reaction-specific, but there is a common root for each type. Thus, for the full implementation of the San Diego mechanism, these roots will be repeated multiple types with variations in e.g., indices and specific parameter values. While these variations are cumbersome in hand implementations, they become meaningless in the context of automated implementations. Thus, we will create a symbolic manipulation engine---termed the symbolic core---that can flexibly manage these small variations.  %Yet, in the context of automated implementations, these variations are insignificant, and this hold even for mechanisms for different fuels.

Another basic aspect that will guide development, diagramed in Figure~\ref{fig:pyro_source_term_eval_sequence}, is the sequence of steps to compute chemical source terms. This basic sequence of steps is independent of chemical mechanism, so specific implementations---e.g., for hydrogen \ce{H2} ($N = 9$ and $M \approx 20$) versus methane \ce{CH4} ($N \gtrsim 30$ and $M \gtrsim 200$) combustion---will have a common structure. This structure will be referred to as the outer shell of the implementation. Together with the symbolic core, it forms a code template.

\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.9,page=1]{Figures/pdf/fig_pyro_source_term_procedure.pdf}
    \caption{High-level representation of source-term evaluation. The symbols are: $\rho$ the density, $T$ the temperature, $\bvec{y}$ the mass fractions, $\bvec{C}$ the concentrations, $\bvec{K}$ the equilibrium constants, $\bvec{k}$ the rate coefficients, $\bvec{R}$ the reaction rates, and $\bvec{\omega}$ the species net production rates.}
    \label{fig:pyro_source_term_eval_sequence}
  \end{center}
\end{figure}


%For now, we will assume that hard-coding Arrhenius parameters is sufficient for subsequent calculations and capabilities.

An example template is provided in Figure~\ref{fig:pyro_template}~(a). The template displays its two main components: the outer shell and symbolic core. The outer shell is structured as a class that remains mostly unchanged upon rendering. Its member functions provide entry points in to the computational implementation of the thermochemistry of Section~\ref{sec:formulation}; specific discussion of these is deferred to Section~\ref{subsub:entrypoints}. The symbolic core creates code for the expressions of the thermochemistry. The core is implemented in \texttt{path/to/pyrometheus/chem\_expr.py}; it encompasses the necessary functionality to generate code for the comprehensive USC-II mechanism, with $N = 111$ species and $M = 784$ reactions~\cite{ref:Wang2007}. Users seeking to implement less conventional expressions (as for ionization or electronic-excitation reactions) can use these as a guide. We discuss the details of the symbolic core next. 

\begin{itemize}
\item Outer shell
  \begin{itemize}
  \item Structured as a class
    \begin{itemize}
    \item For now, suffice to say member variables are gas-phase combustion and mechanism data
    \item Member functions are entrypoints---link between computation and formulation of Section~\ref{sec:formulation}
    \item Specifics deferred to Section~\ref{subsub:entrypoints}, in favor of focused discussion on symbolic generation
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}
\item Symbolic core
  \begin{itemize}
  \item Provides symbolic generation and manipulation
  \item Implementation as a module: \texttt{pyrometheus/chem\_expr.py}
  \item Based on symbolic package Pymbolic
  \item Outputs
  \item Inputs
  \end{itemize}
\end{itemize}



\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.8, page=1]{Figures/pdf/fig_pyro_template.pdf}
    \caption{Pyrometheus (a) code template, and (b) generated code for the San Diego mechanism~\cite{ref:Saxena2006}.}
    \label{fig:pyro_template}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
    \subfloat[][Species net production rate~\eqref{production_rates}.]{\includegraphics[scale=0.8, page=1]{Figures/pdf/fig_pyro_expressions.pdf}}\\
    \subfloat[][Arrhenius rate coefficient~\eqref{rate_coeff}.]{\includegraphics[scale=0.8, page=2]{Figures/pdf/fig_pyro_expressions.pdf}}
    \caption{Expression-generating functions, with examples corresponding to the San Diego mechanism.}
    \label{fig:pyro_expressions}
  \end{center}
\end{figure}

\subsubsection{Pyrometheus Entry Points}\label{subsub:entrypoints}

Next, we discuss entry points that Pyrometheus generated code provides into the thermochemistry: the link between functionality and physical quantities of Section~\ref{sec:formulation}. 

\subsubsection{Array Context}

Loosely following NumPy semantics, the illustrative generated code of Figure~\ref{fig:pyro_template}~(b) implies array-like quantities: in line~{\color{red}9}, the rate of progress \texttt{r} has multiple entries e.g., \texttt{r[4]} and \texttt{r[19]}. Plainly, these represent the rates of progress of reactions 5 and 20, but what exactly these map to depends on the inputs to \texttt{get\_net\_production\_rates}. Were these inputs NumPy arrays of 64-bit floating-point numbers, then each entry of \texttt{r} would map to memory locations of floating-point data for corresponding rates of progress. Alternatively, the inputs could be object arrays representing a more complex data struct such as flow simulation fields discretized on a grid. Yet, in the generated code, there is no unambiguous indication that \texttt{r} is a NumPy array, object or otherwise. 

\begin{itemize}
\item Array context
  \begin{itemize}
  \item Definition
    \begin{itemize}
    \item Semantics of array-valued expressions in Pyrometheus-generated code
    \item NumPy: 
      \begin{itemize}
      \item Follows NumPy syntax and semantics
      \item No floating-point data behind a pointer
      \end{itemize}
    \end{itemize}
  \item Properties and advantages
    \begin{itemize}
    \item Not invasive
    \item Choose from existing contexts after code generation
    \end{itemize}
  \end{itemize}
\end{itemize}

We rely on the notion of an \textit{array context}, which provides the semantics for array-valued expressions in the Pyrometheus-generated code. 

\subsection{Enabled Capabilities}


==> old/outline_design.tex <==
\section{Computational Approach}

\textbf{Goals}

\begin{itemize}
\item Mitigate cost
  \begin{itemize}
  \item Through GPUs     
  \end{itemize}
\item Exact derivatives
  \begin{itemize}
  \item Through AD
  \end{itemize}
\end{itemize}

\textbf{Cost Model}
\begin{itemize}
\item Roofline
  \begin{itemize}
  \item Why?
    \begin{itemize}
    \item Relate performance to memory traffic
    \item Ceilings guide optimization
    \end{itemize}
  \item FLOP counts
    \begin{itemize}
    \item What can we say about these?
    \end{itemize}
  \item How do we measure?
    \begin{itemize}
    \item Thermochemistry involves logarithms and exponentials
    \item How many FLOPs do these entail?
    \end{itemize}
  \item Optimizations
    \begin{itemize}
    \item SIMD as a ceiling
    \item Anticipate SIMD to improve performance for flow simulations
      but\dots
      \begin{itemize}
      \item Other use cases? Explained next
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\textbf{Array-based Computation of the Thermochemistry}
\begin{itemize}
\item Motivation
  \begin{itemize}
  \item Simulate homogeneous vs reactors with flow
  \end{itemize}
\item Computational Challenge
  \begin{itemize}
  \item Grid vs no grid, and libraries
    \begin{itemize}
    \item With grid, operations expressed with loops
      \begin{itemize}
      \item Sure can still optimize? No!
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\textbf{Derivatives}
\begin{itemize}
\item Challenges
\end{itemize}

\textbf{Proposed Approach}
\begin{itemize}
\item Array Context
\item Code Generation
\item code Transformations
  \begin{itemize}
  \item Eager vs Lazy?
  \end{itemize}
\end{itemize}

